GRANDMA and HXMT Observations of GRB 221009A -- the Standard-Luminosity Afterglow of a Hyper-Luminous Gamma-Ray Burst

GRB 221009A is the brightest Gamma-Ray Burst (GRB) detected in more than 50 years of study. In this paper, we present observations in the X-ray and optical domains after the GRB obtained by the GRANDMA Collaboration (which includes observations from more than 30 professional and amateur telescopes) and the Insight-HXMT Collaboration. We study the optical afterglow with empirical fitting from GRANDMA+HXMT data, augmented with data from the literature up to 60 days. We then model numerically, using a Bayesian approach, the GRANDMA and HXMT-LE afterglow observations, that we augment with Swift-XRT and additional optical/NIR observations reported in the literature. We find that the GRB afterglow, extinguished by a large dust column, is most likely behind a combination of a large Milky-Way dust column combined with moderate low-metallicity dust in the host galaxy. Using the GRANDMA+HXMT-LE+XRT dataset, we find that the simplest model, where the observed afterglow is produced by synchrotron radiation at the forward external shock during the deceleration of a top-hat relativistic jet by a uniform medium, fits the multi-wavelength observations only moderately well, with a tension between the observed temporal and spectral evolution. This tension is confirmed when using the extended dataset. We find that the consideration of a jet structure (Gaussian or power-law), the inclusion of synchrotron self-Compton emission, or the presence of an underlying supernova do not improve the predictions, showing that the modelling of GRB22109A will require going beyond the most standard GRB afterglow model. Placed in the global context of GRB optical afterglows, we find the afterglow of GRB 221009A is luminous but not extraordinarily so, highlighting that some aspects of this GRB do not deviate from the global known sample despite its extreme energetics and the peculiar afterglow evolution.

==> GRB221009A - Afterglow - APJL soumission(1)/SED_results.tex <==
\renewcommand{\arraystretch}{1.4}
\begin{longtable}{cccccccc}
    \label{Table:host220427A}
	\caption[Table]{Summary of SED fitting results. (1) stellar mass in log scale, (2) SFR in log scale, (3) amount of dust attenuation in the V band, (4) metallicity, (5) age weighted by stellar mass, (6) attenuation curve slope for stellar continuum, (7) AGN fraction, (8) mass fraction of the late burst population.} \\ \hline
	%\label{tab:GRBHs_results}
    log$_{10}$(M$_{\star}$) & log$_{10}$(SFR) & A$_V$ & $Z$ & t$_{mass}$ & $\delta$ & $f_{agn}$ & $f_{burst}$ \\
    
	[M$_{\sun}$] & [M$_{\sun}$ yr$^{-1}$] & mag & & Myrs & & & \\ \hline
	\endfirsthead %\hline
$10.62_{-0.32}^{+0.18}$ & $1.89_{-nan}^{+0.31}$ & $1.32\pm0.51$ & $0.004_{-0.004}^{+0.007}$ & $802\pm668$ & $-0.60\pm0.30$ & $0.03_{-0.03}^{+0.06}$ & $0.08_{-0.08}^{+0.08}$ \\ \hline

\end{longtable}

==> GRB221009A - Afterglow - APJL soumission(1)/cigal_params.tex <==
\begin{table}
	\renewcommand{\arraystretch}{1.2}
	\centering
	\caption{Input parameters for SED fitting with CIGALE}
	\label{Table:paramshost220427A}
	\begin{tabular}{c c c}
	\hline
	Parameter & Symbol & Range \\
	\hline\hline
	{\textbf{Delayed star formation history $+$ recent burst}}\\
	
	Age of the main stellar population & $t_0$ &  200, 500, 1000, 2000, 3000 \,Myrs \\
	E-folding time of the main stellar population model & $\tau$ &  200, 500, 1000, 2000, 3000, 5000, 7000, 10000  Myrs\\
	Mass fraction of the late burst population & $f_{burst}$ &  0.0, 0.1, 0.2\\
	Age of the late burst & $t_b$ &  20.0, 50.0, 100.0, 200.0\\
	E-folding time of the late starburst population & $\tau_{b}$ &  50.0\\
	%Age of the late starburst population & $t_{\rm b}$ &  1, 3, 5, 10, 15, 20, 30, 40, 50, 75, 100 \,Myrs \\
	%e-folding time of the late starburst population model & $\tau_{\rm b}$ &  50, 50000\,Myrs \\
	%Stellar mass fraction due to the burst & $f_{\rm b}$ &  0, 0.01, 0.03, 0.05, 0.075, 0.1, 0.15, 0.20\\
	\hline
	Metallicity $^1$ & $Z$ & 0.0001, 0.008, 0.02\\
    \hline
	{\textbf{Dust attenuation}}\\
	Color excess for nebular emission $^2$ & $\rm E(B-V)_{lines}$ & 0.01, 0.25, 0.5, 0.75, 1.0, 1.25, 1.5, 1.75, 2.0, 2.25, 2.5, 2.75, 3.0 \\
	Ratio of color excess & $\cfrac{E(B-V)_{stars}}{E(B-V)_{lines}}$ & 0.44 \\
	Attenuation curve slope for stellar continuum & $\delta$ & -1, -0.7, -0.4, -0.1, 0.2, 0.5, 0.7\\
	\hline
	{\textbf{AGN$^4$}}\\
	Slope of the power law & $\alpha$ & 2.0\\
	AGN fraction & $f_{agn}$ & 0.0, 0.1, 0.2 \\
	\hline
	Redshift & $z$ & 0.8159 \\
	\hline	
	\hline
	\end{tabular}
	\begin{flushleft}
      \small
      \item $^1$ {$Z$=0.02 being the solar metallicity}
      \item $^2$ {$\rm E(B-V)_{lines}$ is the color excess between the B and V bands applied on the nebular emission lines.}
      \item $^3$ {M$_d$ corresponds to the dust mass heated by the the radiation field intensity U. $\alpha_{IR}$ is fixed to 2 when no IR detection is available.}
      \item $^4$ {Parameters of the dale2014 model \cite{Boquien2019}.}
    \end{flushleft}

\end{table}

==> GRB221009A - Afterglow - APJL soumission(1)/datatab1.tex <==
\begin{table*}
\caption{Data used for the numerical data analysis sections (\S\ref{NMMA}, \S\ref{IAP}). \textit{Swift} data have been converted from the Vega system to the AB system. Data are given fully extinction-corrected, for either SF11 MW foreground extinction (described in section~\ref{SED}, or RF09\footnote{This does not include updated measurements provided after Feb. 05. 2022}, and the corresponding SMC extinction in the host galaxy (\S\ref{SED}).}
\label{tab:GRANDMA_observations}
\scalebox{0.9}{
\begin{tabular}{|cc|c|cc|cc|c|}
\hline
\multicolumn{2}{|c|}{Delay} & Filter &  \multicolumn{2}{c|}{SF11}  & \multicolumn{2}{c|}{RF09} & Observatory \\
  (day) & (sec)  &  & Magnitude  & Upper-limit & Magnitude  & Upper-limit & \\
\hline
%\multicolumn{8}{c}{X-ray} \\
%\hline
%0.0487	& $4.209\times10^3$  & $uvw2$ &  - & 9.15 &  - & 14.72 & \textit{Swift} UVOT \\
%\hline
%0.0485	& $4.190\times10^3$ & $uvw1$ & $11.73^{+0.61}_{-0.39}$ & - & $15.86^{+0.61}_{-0.39}$ & -  & \textit{Swift} UVOT \\
%\hline
0.0423 & $3.657\times10^3$ & $u$ & $10.87\pm0.15$ & - & $10.65\pm0.35$ & - & \textit{Swift} UVOT \\	 
0.0457 & $3.949\times10^3$ & $u$ & $11.03\pm0.30$` & - & $10.77\pm0.44$ & -  & \textit{Swift} UVOT \\
0.0511 & $4.416\times10^3$ & $u$ & $10.91\pm0.22$ & - & $10.75\pm0.39$  & - & \textit{Swift} UVOT \\
0.3755 & $3.244\times10^4$ & $u$ & $13.40\pm0.22$ & - & - & - & \textit{Swift} UVOT \\
0.5751 & $4.969\times10^4$ & $u$ & $13.88\pm0.30$ & - & - & - & \textit{Swift} UVOT \\
1.1084 & $9.576\times10^4$ & $u$ & $14.25\pm0.39$ & - & - & - & \textit{Swift} UVOT \\

\hline
%0.0440 & $3.800\times10^3$ & $b$ & $11.47^{+0.13}_{-0.11}$ & - & $13.98^{+0.13}_{-0.11}$ & - & \textit{Swift} UVOT \\
%0.0460 & $3.973\times10^3$ & $b$ & $11.59^{+0.14}_{-0.12}$ & - & $14.10^{+0.14}_{-0.12}$ & -  & \textit{Swift} UVOT \\
%0.0513 & $4.436\times10^3$ & $b$ & $11.88^{+0.13}_{-0.12}$ & - & $14.40^{+0.13}_{-0.12}$  & - & \textit{Swift} UVOT \\
%\hline
%0.0448 & $3.875\times10^3$ & $v$ & $11.32^{+0.11}_{-0.10}$ & - & $13.28^{+0.11}_{-0.10}$  & - & \textit{Swift} UVOT \\
%0.0469 & $4.048\times10^3$ & $v$ & $11.33^{+0.11}_{-0.10}$ & - & $13.29^{+0.11}_{-0.10}$  & - & \textit{Swift} UVOT \\
%0.0503 & $4.342\times10^3$ & $v$ & $11.58^{+0.09}_{-0.08}$ & - & $13.54^{+0.09}_{-0.08}$  & - & \textit{Swift} UVOT \\
%\hline
%0.0399 & $3.450\times10^3$ & $white$ & $10.84^{+0.02}_{-0.02}$ & - & $13.97^{+0.02}_{-0.02}$  & - & \textit{Swift} UVOT \\
%0.0443 & $3.824\times10^3$ & $white$ & $10.86^{+0.06}_{-0.06}$ & - & $14.00^{+0.06}_{-0.06}$  & - & \textit{Swift} UVOT \\
%0.0463 & $3.998\times10^3$ & $white$ & $11.11^{+0.07}_{-0.07}$ & - & $14.24^{+0.07}_{-0.07}$  & - & \textit{Swift} UVOT \\
%0.0479 & $4.141\times10^3$ & $white$ & $11.08^{+0.02}_{-0.03}$ & - & $14.21^{+0.02}_{-0.03}$  & - & \textit{Swift} UVOT \\
%0.0507 & $4.379\times10^3$ & $white$ & $11.10^{+0.07}_{-0.07}$ & - & $14.23^{+0.07}_{-0.07}$  & - & \textit{Swift} UVOT \\
%0.2530 & $2.186\times10^4$ & $white$ & $12.90^{+0.04}_{-0.04}$ & - & $16.04^{+0.04}_{-0.04}$  & - & \textit{Swift} UVOT  \\ 
%\hline
0.2572 & $2.222\times10^4$ & $B$ & - & 11.76 & - & 11.69 & KNC-SCT-0.28  \\ 
\hline
 1.1368 & $9.822\times10^4$ & $g^\prime$ & $14.81\pm0.21$ & - & $14.70\pm0.31$  & - & KAO  \\ 
 19.6945  & $1.702\times10^6$ & $g^\prime$ & $18.95\pm0.22$ & - & $18.84\pm0.31$ & - & CFHT-Megacam \\ 
\hline
-0.0010 &    -90 & $V$ & - & -2.79 &  - & -2.9 & Mundrabilla \\
-0.0007 &    -60 & $V$ & - & -2.79 &  - & -2.9 & Mundrabilla \\
-0.0003 &    -30 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0000 &       0 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0004 &      30 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0007 &      60 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0011 &      90 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0014 &     120 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0017 &     150 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0021 &     180 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0024 &     210 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0031 &     270 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0035 &     300 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0042 &     360 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.0045 &     390 & $V$ & - & -0.99 &  - & -1.1 & Raw War Road \\
0.2677 & $2.313\times10^4$ & $V$ & $12.60\pm0.10$ & - & $12.50\pm0.22$  & - & KNC-SCT-0.28 \\ 
1.1465 & $9.906\times10^4$ & $V$ & $14.57\pm0.16$ & - &  $14.47\pm0.26$ & - & ShAO \\
1.2606 & $1.089\times10^5$ & $V$ &  -  & 13.90 &   - & 13.80 & KNC-SCT-0.28 \\
\hline
0.0972 & $8.40\times10^3$ & $r^\prime$ & $11.90\pm0.13$ & - &  $11.79\pm0.21$ & - & TRE \\
0.0993 & $8.58\times10^3$ & $r^\prime$ & $11.80\pm0.19$ & - & $11.69\pm0.25$ & - & TRE  \\
0.0995 & $8.60\times10^3$ & $r^\prime$  & $11.72\pm0.29$ & - & $11.61\pm0.33$ & - & TRE \\
0.1748 & $1.510\times10^4$ & $r^\prime$ & $12.38\pm0.31$ & - & $12.27\pm0.35$ & - & TRE \\
0.1750 & $1.512\times10^4$ & $r^\prime$ & $11.86\pm0.24$ & - & $11.75\pm0.29$ & - & TRE  \\
1.1489 & $9.926\times10^4$ & $r^\prime$  & $14.63\pm0.10$ & - & $14.52\pm0.19$ & - & KAO \\
1.3077 & $1.130\times10^5$ & $r^\prime$ & $14.84\pm0.07$ &  - & $14.73\pm0.18$ & - & C2PU/Omicron  \\
2.3083 & $1.994\times10^5$ & $r^\prime$ &  $15.34\pm0.16$  & - &  $15.23\pm0.23$ & - & KNC-Parent \\
2.5206 & $2.178\times10^5$ & $r^\prime$ &  $15.54\pm0.13$ & - & $15.43\pm0.21$  & - &  KNC-LCO/McDO-0.4m \\
3.2874 & $2.840\times10^5$ & $r^\prime$ &  -  & 14.38 &  - & 14.27 &  KNC-C11-ATLAS \\
4.2097 & $3.637\times10^5$ & $r^\prime$ & - & 16.18 & -  & 16.07 & KAO  \\
10.2667  & $8.870\times10^5$ & $r^\prime$ & $17.74\pm0.09$ & - & $17.63\pm0.19$ & - & C2PU/Omicron \\
19.6965 & $1.702\times10^6$ & $r^\prime$ & $18.67\pm0.07$ & - & $18.56\pm0.18$ & - & CFHT/MegaCam \\
 \hline
 0.2736 & $2.364\times10^4$ & $R_C$ & $12.41\pm0.07$ & - & $12.34\pm0.18$ & - & KNC-SCT-0.28 \\
1.0813 & $9.342\times10^4$ & $R_C$ & $14.36\pm0.15$ & - & $14.29\pm0.22$ & - & UBAI-ST60  \\
 1.2274 & $1.060\times10^5$ & $R_C$ & $14.25\pm0.10$ & - & $14.18\pm0.19$ & - & Lisnyky AZT-8   \\
 1.2365 & $1.068\times10^5$ & $R_C$ & $14.39\pm0.10$ & - & $14.32\pm0.19$ & - & Lisnyky AZT-8   \\
1.2755 & $1.102\times10^5$ & $R_C$ & - & 14.30 & - & 14.23 & KNC-SCT-0.28 \\
2.2956 & $1.983\times10^5$ & $R_C$ & - & 14.91 & - & 14.84 & KNC-SCT-0.28 \\
\hline
\end{tabular}}
\end{table*}

\begin{table*}
\addtocounter{table}{-1}
\caption{Continued.}
\scalebox{0.9}{
\begin{tabular}{|cc|c|cc|cc|c|}
\multicolumn{2}{|c|}{Delay} & Filter &  \multicolumn{2}{c|}{SF11}  & \multicolumn{2}{c|}{RF09} & Observatory \\
  (day) & (sec)  &  & Magnitude  & Upper-limit & Magnitude  & Upper-limit & \\
\hline
2.3042  & $1.991\times10^5$ & $R_C$ & $15.37\pm0.10$ & - & $15.30\pm0.19$ & - & Lisnyky AZT-8  \\
3.2868  & $2.840\times10^5$ & $R_C$ & $16.13\pm0.12$ & - &  $16.06\pm0.20$ & - & Lisnyky AZT-8  \\
5.0674 & $4.378\times10^5$ & $R_C$ & - & 14.61 & - & 14.54 &  UBAI-ST60 \\
11.1313 & $9.617\times10^5$ & $R_C$  & $18.01\pm0.19$ & - & $17.94\pm0.25$ & - & UBAI-AZT22 \\
12.4567 & $1.076\times10^6$ & $R_C$ & - & 16.02 & - & 15.95 & VIRT \\
\hline
0.5333 & $4.608\times10^4$ & $i^\prime$ & $13.20\pm0.06$  & - &  $13.13\pm0.14$  & - &  KNC-BGO \\
0.5372 & $4.641\times10^4$ & $i^\prime$ & $13.21\pm0.06$  & - &  $13.14\pm0.14$  & - &  KNC-BGO \\
0.5411 & $4.675\times10^4$ & $i^\prime$ & $13.24\pm0.06$  & - &  $13.17\pm0.14$  & - &  KNC-BGO \\
0.5450 & $4.709\times10^4$ & $i^\prime$ & $13.30\pm0.06$  & - &  $13.23\pm0.14$  & - &  KNC-BGO \\
0.5489 & $4.742\times10^4$ & $i^\prime$ & $13.34\pm0.07$  & - &  $13.27\pm0.15$  & - &  KNC-BGO \\
0.5527 & $4.775\times10^4$ & $i^\prime$ & $13.33\pm0.06$  & - &  $13.26\pm0.14$  & - &  KNC-BGO \\
0.5572 & $4.814\times10^4$ & $i^\prime$ & $13.42\pm0.06$  & - &  $13.35\pm0.14$  & - &  KNC-BGO \\
0.5611 & $4.848\times10^4$ & $i^\prime$ & $13.40\pm0.06$  & - &  $13.33\pm0.14$  & - &  KNC-BGO \\
0.5650 & $4.882\times10^4$ & $i^\prime$ & $13.37\pm0.07$  & - &  $13.30\pm0.15$  & - &  KNC-BGO \\
0.5689 & $4.915\times10^4$ & $i^\prime$ & $13.23\pm0.06$ & - & $13.16\pm0.14$ & - &  KNC-BGO \\
0.5727 & $4.948\times10^4$ & $i^\prime$ & $13.40\pm0.07$ & - & $13.33\pm0.15$ & - &  KNC-BGO \\
0.5766 & $4.982\times10^4$ & $i^\prime$ & $13.54\pm0.08$ & - & $13.47\pm0.15$ & - &  KNC-BGO \\
1.1625 & $1.004\times10^5$ & $i^\prime$ & $14.63\pm0.06$ & - & $14.56\pm0.14$ & - & KAO \\
1.2255 & $1.059\times10^5$ & $i^\prime$ &  $14.37\pm0.10$  & - &   $14.30\pm0.16$  & - &  KNC-IRIS \\
2.5092 & $2.168\times10^5$ & $i^\prime$ & $15.40\pm0.10$  & - &   $15.33\pm0.16$  & - &  KNC-BGO \\
3.5534 & $3.070\times10^5$ & $i^\prime$ &  $16.46\pm0.22$  & - &   $16.39\pm0.26$  & - &  KNC-BGO \\
4.2108 & $3.638\times10^5$ & $i^\prime$ & $16.69\pm0.30$ & - & $16.62\pm0.33$ & - & KAO \\
19.7097  & $1.703\times10^6$ & $i^\prime$  & $18.83\pm0.06$ & - & $18.76\pm0.14$ & - & CFHT/MegaCam  \\
\hline
0.2887 & $2.494\times10^4$ & $I_C$ &  $12.40\pm0.06$  & - &   $12.21\pm0.13$  & - &  KNC-SCT-0.28 \\
1.2902 & $1.115\times10^5$ & $I_C$ &  $14.31\pm0.14$  & - &   $14.12\pm0.18$  & - &  KNC-SCT-0.28 \\
2.3509 & $2.031\times10^5$ & $I_C$ &  -  & 14.79 &   -  & 14.60 &  KNC-SCT-0.28 \\
6.3104 & $5.452\times10^5$ & $I_C$ & $16.96\pm0.17$ & - &  $16.77\pm0.21$ & - & Lisnyky AZT-8 \\
15.4848 & $1.338\times10^6$ & $I_C$ & - & 16.98 & - & 16.79 & VIRT \\
\hline
1.1745 & $1.015\times10^5$ & $z^\prime$  &  $14.80\pm0.07$ & - & $14.70\pm0.11$ & - & KAO \\
4.217 & $3.643\times10^5$ & $z^\prime$  &  $16.73\pm0.16$ & - & $16.63\pm0.19$ & - & KAO \\
13.184 & $1.139\times10^6$ & $z^\prime$  &  - & 18.23 & - & 18.13 & KAO \\
19.7308  & $1.705\times10^6$ & $z^\prime$ & $18.84\pm0.09$ & - & $18.74\pm0.12$ & - &  CFHT/MegaCam \\
\hline
\multicolumn{2}{|c|}{Delay} & X-ray Filter &  \multicolumn{2}{c|}{Flux}  & \multicolumn{2}{c|}{Flux error} & Observatory \\
  (day) & (sec)  & Central frequency & \multicolumn{2}{c|}{(Jansky)} & \multicolumn{2}{c|}{(Jansky)} & \\
\hline
0.1644 & $1.420\times10^4$ & 5 keV & \multicolumn{2}{c|}{$3.74\times 10^{-4}$} & \multicolumn{2}{c|}{$7.49\times 10^{-5}$} & \textit{HXMT}/LE \\
0.3617 & $3.125\times10^4$ & 5 keV & \multicolumn{2}{c|}{$9.32\times 10^{-5}$} & \multicolumn{2}{c|}{$2.06\times 10^{-5}$} & \textit{HXMT}/LE \\
0.8580 & $7.413\times10^4$ & 5 keV & \multicolumn{2}{c|}{$1.83\times 10^{-5}$} & \multicolumn{2}{c|}{$3.66\times 10^{-6}$} & \textit{HXMT}/LE \\
0.9896 & $8.550\times10^4$ & 5 keV & \multicolumn{2}{c|}{$1.49\times 10^{-5}$} & \multicolumn{2}{c|}{$2.99\times 10^{-6}$} & \textit{HXMT}/LE \\
1.1223 & $9.697\times10^4$ & 5 keV & \multicolumn{2}{c|}{$1.23\times 10^{-5}$} & \multicolumn{2}{c|}{$2.45\times 10^{-6}$} & \textit{HXMT}/LE \\
1.2192 & $1.053\times10^5$ & 5 keV & \multicolumn{2}{c|}{$1.41\times 10^{-5}$} & \multicolumn{2}{c|}{$5.53\times 10^{-6}$} & \textit{HXMT}/LE \\
1.3864 & $1.198\times10^5$ & 5 keV & \multicolumn{2}{c|}{$7.18\times 10^{-6}$} & \multicolumn{2}{c|}{$1.44\times 10^{-6}$} & \textit{HXMT}/LE \\
1.5256 & $1.318\times10^5$ & 5 keV & \multicolumn{2}{c|}{$6.17\times 10^{-6}$} & \multicolumn{2}{c|}{$1.23\times 10^{-6}$} & \textit{HXMT}/LE \\
1.6526 & $1.428\times10^5$ & 5 keV & \multicolumn{2}{c|}{$5.45\times 10^{-6}$} & \multicolumn{2}{c|}{$1.09\times 10^{-6}$} & \textit{HXMT}/LE \\
1.7844 & $1.542\times10^5$ & 5 keV & \multicolumn{2}{c|}{$4.44\times 10^{-6}$} & \multicolumn{2}{c|}{$8.87\times 10^{-7}$} & \textit{HXMT}/LE \\
1.9157 & $1.655\times10^5$ & 5 keV & \multicolumn{2}{c|}{$3.91\times 10^{-6}$} & \multicolumn{2}{c|}{$7.82\times 10^{-7}$} & \textit{HXMT}/LE \\
2.0485 & $1.770\times10^5$ & 5 keV & \multicolumn{2}{c|}{$3.91\times 10^{-6}$} & \multicolumn{2}{c|}{$8.87\times 10^{-7}$} & \textit{HXMT}/LE \\
2.1473 & $1.855\times10^5$ & 5 keV & \multicolumn{2}{c|}{$2.19\times 10^{-6}$} & \multicolumn{2}{c|}{$7.59\times 10^{-7}$} & \textit{HXMT}/LE \\
2.4809 & $2.143\times10^5$ & 5 keV & \multicolumn{2}{c|}{$3.73\times 10^{-6}$} & \multicolumn{2}{c|}{$1.93\times 10^{-6}$} & \textit{HXMT}/LE \\
2.5822 & $2.231\times10^5$ & 5 keV & \multicolumn{2}{c|}{$1.92\times 10^{-6}$} & \multicolumn{2}{c|}{$3.84\times 10^{-7}$} & \textit{HXMT}/LE \\
2.7138 & $2.345\times10^5$ & 5 keV & \multicolumn{2}{c|}{$3.64\times 10^{-6}$} & \multicolumn{2}{c|}{$2.62\times 10^{-6}$} & \textit{HXMT}/LE \\
2.8464 & $2.459\times10^5$ & 5 keV & \multicolumn{2}{c|}{$3.73\times 10^{-6}$} & \multicolumn{2}{c|}{$3.83\times 10^{-6}$} & \textit{HXMT}/LE \\
2.9744 & $2.570\times10^5$ & 5 keV & \multicolumn{2}{c|}{$1.27\times 10^{-6}$} & \multicolumn{2}{c|}{$8.57\times 10^{-7}$} & \textit{HXMT}/LE \\
\hline
\end{tabular}}
\end{table*}

\begin{table*}
\addtocounter{table}{-1}
\caption{Continued.}
\scalebox{0.9}{
\begin{tabular}{|cc|c|cc|cc|c|}
\multicolumn{2}{|c|}{Delay} & X-ray Filter &  \multicolumn{2}{c|}{Flux}  & \multicolumn{2}{c|}{Flux error} & Observatory \\
  (day) & (sec)  & Central frequency & \multicolumn{2}{c|}{(Jansky)} & \multicolumn{2}{c|}{(Jansky)} & \\
\hline
0.0419 & $0.362\times10^4$  & 10 keV & \multicolumn{2}{c|}{$1.23\times 10^{-3}$} & \multicolumn{2}{c|}{$2.51\times 10^{-4}$} & \textit{Swift} XRT \\
0.0486 & $0.420\times10^4$  & 10 keV & \multicolumn{2}{c|}{$8.95\times 10^{-4}$} & \multicolumn{2}{c|}{$1.88\times 10^{-4}$} & \textit{Swift} XRT \\
0.2529 & $2.185\times10^4$  & 10 keV & \multicolumn{2}{c|}{$7.23\times 10^{-5}$} & \multicolumn{2}{c|}{$2.14\times 10^{-5}$} & \textit{Swift} XRT \\
0.3018 & $2.608\times10^4$  & 10 keV & \multicolumn{2}{c|}{$5.71\times 10^{-5}$} & \multicolumn{2}{c|}{$1.64\times 10^{-5}$} & \textit{Swift} XRT \\
0.3701 & $3.197\times10^4$  & 10 keV & \multicolumn{2}{c|}{$3.76\times 10^{-5}$} & \multicolumn{2}{c|}{$1.10\times 10^{-5}$} & \textit{Swift} XRT \\
0.4365 & $3.771\times10^4$  & 10 keV & \multicolumn{2}{c|}{$3.29\times 10^{-5}$} & \multicolumn{2}{c|}{$9.87\times 10^{-6}$} & \textit{Swift} XRT \\
0.5145 & $4.445\times10^4$  & 10 keV & \multicolumn{2}{c|}{$2.87\times 10^{-5}$} & \multicolumn{2}{c|}{$9.62\times 10^{-6}$} & \textit{Swift} XRT \\
0.5698 & $4.923\times10^4$  & 10 keV & \multicolumn{2}{c|}{$1.85\times 10^{-5}$} & \multicolumn{2}{c|}{$6.31\times 10^{-6}$} & \textit{Swift} XRT \\
0.6348 & $5.484\times10^4$  & 10 keV & \multicolumn{2}{c|}{$1.80\times 10^{-5}$} & \multicolumn{2}{c|}{$5.48\times 10^{-6}$} & \textit{Swift} XRT \\
0.7026 & $6.070\times10^4$  & 10 keV & \multicolumn{2}{c|}{$1.22\times 10^{-5}$} & \multicolumn{2}{c|}{$4.97\times 10^{-6}$} & \textit{Swift} XRT \\
0.7808 & $6.746\times10^4$  & 10 keV & \multicolumn{2}{c|}{$1.22\times 10^{-5}$} & \multicolumn{2}{c|}{$4.72\times 10^{-6}$} & \textit{Swift} XRT \\
0.8481 & $7.327\times10^4$  & 10 keV & \multicolumn{2}{c|}{$1.06\times 10^{-5}$} & \multicolumn{2}{c|}{$3.63\times 10^{-6}$} & \textit{Swift} XRT \\
1.0395 & $8.982\times10^4$  & 10 keV & \multicolumn{2}{c|}{$8.91\times 10^{-6}$} & \multicolumn{2}{c|}{$3.54\times 10^{-6}$} & \textit{Swift} XRT \\
1.2431 & $1.074\times10^5$  & 10 keV & \multicolumn{2}{c|}{$7.61\times 10^{-6}$} & \multicolumn{2}{c|}{$2.45\times 10^{-6}$} & \textit{Swift} XRT \\
1.4247 & $1.231\times10^5$  & 10 keV & \multicolumn{2}{c|}{$5.73\times 10^{-6}$} & \multicolumn{2}{c|}{$1.91\times 10^{-6}$} & \textit{Swift} XRT \\
1.6254 & $1.404\times10^5$  & 10 keV & \multicolumn{2}{c|}{$3.77\times 10^{-6}$} & \multicolumn{2}{c|}{$1.48\times 10^{-6}$} & \textit{Swift} XRT \\
1.8796 & $1.624\times10^5$  & 10 keV & \multicolumn{2}{c|}{$3.36\times 10^{-6}$} & \multicolumn{2}{c|}{$1.17\times 10^{-6}$} & \textit{Swift} XRT \\
2.5980 & $2.245\times10^5$  & 10 keV & \multicolumn{2}{c|}{$2.32\times 10^{-6}$} & \multicolumn{2}{c|}{$5.38\times 10^{-7}$} & \textit{Swift} XRT \\
2.8842 & $2.492\times10^5$  & 10 keV & \multicolumn{2}{c|}{$1.37\times 10^{-6}$} & \multicolumn{2}{c|}{$3.63\times 10^{-7}$} & \textit{Swift} XRT \\
3.4783 & $3.005\times10^5$  & 10 keV & \multicolumn{2}{c|}{$1.02\times 10^{-6}$} & \multicolumn{2}{c|}{$3.60\times 10^{-7}$} & \textit{Swift} XRT \\
4.5403 & $3.923\times10^5$  & 10 keV & \multicolumn{2}{c|}{$7.20\times 10^{-7}$} & \multicolumn{2}{c|}{$2.87\times 10^{-7}$} & \textit{Swift} XRT \\
5.6807 & $4.908\times10^5$  & 10 keV & \multicolumn{2}{c|}{$4.04\times 10^{-7}$} & \multicolumn{2}{c|}{$1.46\times 10^{-7}$} & \textit{Swift} XRT \\
7.1565 & $6.183\times10^5$  & 10 keV & \multicolumn{2}{c|}{$2.85\times 10^{-7}$} & \multicolumn{2}{c|}{$1.28\times 10^{-7}$} & \textit{Swift} XRT \\
9.5104 & $8.217\times10^5$  & 10 keV & \multicolumn{2}{c|}{$1.37\times 10^{-7}$} & \multicolumn{2}{c|}{$6.70\times 10^{-8}$} & \textit{Swift} XRT \\
13.260 & $1.146\times10^6$  & 10 keV & \multicolumn{2}{c|}{$7.76\times 10^{-8}$} & \multicolumn{2}{c|}{$2.97\times 10^{-8}$} & \textit{Swift} XRT \\
18.832 & $1.627\times10^6$  & 10 keV & \multicolumn{2}{c|}{$4.86\times 10^{-8}$} & \multicolumn{2}{c|}{$1.31\times 10^{-8}$} & \textit{Swift} XRT \\
28.236 & $2.440\times10^6$  & 10 keV & \multicolumn{2}{c|}{$2.21\times 10^{-8}$} & \multicolumn{2}{c|}{$8.34\times 10^{-9}$} & \textit{Swift} XRT \\
41.971 & $3.626\times10^6$  & 10 keV & \multicolumn{2}{c|}{$1.48\times 10^{-8}$} & \multicolumn{2}{c|}{$3.81\times 10^{-9}$} & \textit{Swift} XRT \\
64.598 & $5.581\times10^6$  & 10 keV & \multicolumn{2}{c|}{$2.59\times 10^{-9}$} & \multicolumn{2}{c|}{$1.23\times 10^{-9}$} & \textit{Swift} XRT \\
\hline
0.0419 & $0.362\times10^4$  & 1 keV & \multicolumn{2}{c|}{$8.36\times 10^{-3}$} & \multicolumn{2}{c|}{$1.16\times 10^{-3}$} & \textit{Swift} XRT \\
0.0486 & $0.420\times10^4$  & 1 keV & \multicolumn{2}{c|}{$7.25\times 10^{-3}$} & \multicolumn{2}{c|}{$1.04\times 10^{-3}$} & \textit{Swift} XRT \\
0.2529 & $2.185\times10^4$  & 1 keV & \multicolumn{2}{c|}{$5.98\times 10^{-4}$} & \multicolumn{2}{c|}{$1.12\times 10^{-4}$} & \textit{Swift} XRT \\
0.3018 & $2.608\times10^4$  & 1 keV & \multicolumn{2}{c|}{$4.39\times 10^{-4}$} & \multicolumn{2}{c|}{$8.75\times 10^{-5}$} & \textit{Swift} XRT \\
0.3701 & $3.197\times10^4$  & 1 keV & \multicolumn{2}{c|}{$3.59\times 10^{-4}$} & \multicolumn{2}{c|}{$6.76\times 10^{-5}$} & \textit{Swift} XRT \\
0.4365 & $3.771\times10^4$  & 1 keV & \multicolumn{2}{c|}{$2.30\times 10^{-4}$} & \multicolumn{2}{c|}{$5.15\times 10^{-5}$} & \textit{Swift} XRT \\
0.5145 & $4.445\times10^4$  & 1 keV & \multicolumn{2}{c|}{$1.89\times 10^{-4}$} & \multicolumn{2}{c|}{$4.82\times 10^{-5}$} & \textit{Swift} XRT \\
0.5698 & $4.923\times10^4$  & 1 keV & \multicolumn{2}{c|}{$1.91\times 10^{-4}$} & \multicolumn{2}{c|}{$4.60\times 10^{-5}$} & \textit{Swift} XRT \\
0.6348 & $5.484\times10^4$  & 1 keV & \multicolumn{2}{c|}{$1.49\times 10^{-4}$} & \multicolumn{2}{c|}{$3.07\times 10^{-5}$} & \textit{Swift} XRT \\
0.7026 & $6.070\times10^4$  & 1 keV & \multicolumn{2}{c|}{$1.65\times 10^{-4}$} & \multicolumn{2}{c|}{$4.62\times 10^{-5}$} & \textit{Swift} XRT \\
0.7808 & $6.746\times10^4$  & 1 keV & \multicolumn{2}{c|}{$1.19\times 10^{-4}$} & \multicolumn{2}{c|}{$3.07\times 10^{-5}$} & \textit{Swift} XRT \\
0.8481 & $7.327\times10^4$  & 1 keV & \multicolumn{2}{c|}{$9.98\times 10^{-5}$} & \multicolumn{2}{c|}{$2.10\times 10^{-5}$} & \textit{Swift} XRT \\
1.0395 & $8.982\times10^4$  & 1 keV & \multicolumn{2}{c|}{$7.24\times 10^{-5}$} & \multicolumn{2}{c|}{$2.33\times 10^{-5}$} & \textit{Swift} XRT \\
1.2431 & $1.074\times10^5$  & 1 keV & \multicolumn{2}{c|}{$3.96\times 10^{-5}$} & \multicolumn{2}{c|}{$1.23\times 10^{-5}$} & \textit{Swift} XRT \\
1.4247 & $1.231\times10^5$  & 1 keV & \multicolumn{2}{c|}{$3.28\times 10^{-5}$} & \multicolumn{2}{c|}{$8.30\times 10^{-6}$} & \textit{Swift} XRT \\
1.6254 & $1.404\times10^5$  & 1 keV & \multicolumn{2}{c|}{$2.71\times 10^{-5}$} & \multicolumn{2}{c|}{$7.93\times 10^{-6}$} & \textit{Swift} XRT \\
1.8796 & $1.624\times10^5$  & 1 keV & \multicolumn{2}{c|}{$2.28\times 10^{-5}$} & \multicolumn{2}{c|}{$7.84\times 10^{-6}$} & \textit{Swift} XRT \\
2.5980 & $2.245\times10^5$  & 1 keV & \multicolumn{2}{c|}{$1.35\times 10^{-5}$} & \multicolumn{2}{c|}{$2.94\times 10^{-6}$} & \textit{Swift} XRT \\
2.8842 & $2.492\times10^5$  & 1 keV & \multicolumn{2}{c|}{$1.28\times 10^{-5}$} & \multicolumn{2}{c|}{$2.86\times 10^{-6}$} & \textit{Swift} XRT \\
3.4783 & $3.005\times10^5$  & 1 keV & \multicolumn{2}{c|}{$8.41\times 10^{-6}$} & \multicolumn{2}{c|}{$2.59\times 10^{-6}$} & \textit{Swift} XRT \\
4.5403 & $3.923\times10^5$  & 1 keV & \multicolumn{2}{c|}{$5.56\times 10^{-6}$} & \multicolumn{2}{c|}{$1.75\times 10^{-6}$} & \textit{Swift} XRT \\
5.6807 & $4.908\times10^5$  & 1 keV & \multicolumn{2}{c|}{$5.08\times 10^{-6}$} & \multicolumn{2}{c|}{$1.24\times 10^{-6}$} & \textit{Swift} XRT \\
7.1565 & $6.183\times10^5$  & 1 keV & \multicolumn{2}{c|}{$3.77\times 10^{-6}$} & \multicolumn{2}{c|}{$1.16\times 10^{-6}$} & \textit{Swift} XRT \\
9.5104 & $8.217\times10^5$  & 1 keV & \multicolumn{2}{c|}{$2.34\times 10^{-6}$} & \multicolumn{2}{c|}{$5.99\times 10^{-7}$} & \textit{Swift} XRT \\
13.260 & $1.146\times10^6$  & 1 keV & \multicolumn{2}{c|}{$1.27\times 10^{-6}$} & \multicolumn{2}{c|}{$2.92\times 10^{-7}$} & \textit{Swift} XRT \\
18.832 & $1.627\times10^6$  & 1 keV & \multicolumn{2}{c|}{$6.52\times 10^{-7}$} & \multicolumn{2}{c|}{$2.28\times 10^{-7}$} & \textit{Swift} XRT \\
28.236 & $2.440\times10^6$  & 1 keV & \multicolumn{2}{c|}{$4.15\times 10^{-7}$} & \multicolumn{2}{c|}{$1.38\times 10^{-7}$} & \textit{Swift} XRT \\
41.971 & $3.626\times10^6$  & 1 keV & \multicolumn{2}{c|}{$2.59\times 10^{-7}$} & \multicolumn{2}{c|}{$8.25\times 10^{-8}$} & \textit{Swift} XRT \\
64.598 & $5.581\times10^6$  & 1 keV & \multicolumn{2}{c|}{$1.96\times 10^{-7}$} & \multicolumn{2}{c|}{$4.82\times 10^{-8}$} & \textit{Swift} XRT \\

\hline
\end{tabular}}
\end{table*}




==> GRB221009A - Afterglow - APJL soumission(1)/datatab2.tex <==
\begin{center}

\begin{table*}
\caption{The GRANDMA and GCN optical observations of GRB 221009A. In column (2), the $\mathrm{T_{mid}}$ time is the delay between the beginning of the observation and the \textit{Fermi} GBM GRB trigger time (2022-10-09T13:16:59.99) in days. In column (5), magnitudes are given in the AB system and not corrected for Galactic and host-galaxy dust extinction. In column (9), the VETO tag refers to GRANDMA data that were not analyzed due to the bad quality of the images.}
\label{tab:all_observations}
\scalebox{0.6}{
\begin{tabular}{|l|cc|c|l|l|l|c|c|c|}
\hline
\multicolumn{1}{|c|}{T$_{start}$}  & \multicolumn{2}{c|}{T$_{mid}$ (days)}& Filter & Exposure & \multicolumn{1}{c|}{Magnitude} & \multicolumn{1}{c|}{U.L.} & Telescope & Reference & Analysis method \\
\multicolumn{1}{|c|}{UT} & MJD & T-T$_{GRB}$ &  &  &  &  & & & \\
\multicolumn{1}{|c|}{(1)} & \multicolumn{2}{c|}{(2)} & (3) & \multicolumn{1}{|c|}{(4)} & \multicolumn{1}{|c|}{(5)} & \multicolumn{1}{|c|}{(6)} & (7) & (8) & (9) \\
\hline
\hline
2022-10-09T18:06:27	&	59861.7545                	&	0.2010             	&	$u^\prime$ 	&	6$\times$60s       & -	&	17.9 (3$\sigma$)   	&	MeerLICHT      & \cite{2022GCN.32646....1D}   &   -    \\ %ok
2022-10-10T05:00	&	59862.2083                    	&	0.6549 &	$u^\prime$ 	&	6$\times$60s      & -  & -	&	Nickel-1m       & \cite{2022GCN.32669....1V}       &   -  \\ %need to reupdate
\hline
%2022-10-09T19:21	&	59861.8062                    	&	0.2528              	&	$B$     	&	5$\times$180 s & -	&	17.8  	&	\textcolor{black}{KNC-SCT-0.28}   & \cite{2022GCN.32640....1B} \& this work   & APASS DR9 \DT{ from PS1 converted into Johnson B using the transformation in https://ar$\times$iv.org/pdf/2205.06186.pdf}               \\ % Damien tu peu$\times$ refaire l'analyse stp ?
2022-10-09T19:19:51	&	59861.8107       	&	0.2572              	&	$B$     	&	5$\times$180s & -	& 18.1 (5$\sigma$) &	\textcolor{black}{KNC-SCT-0.28}   & \cite{2022GCN.32640....1B} \& this work & \sc{STDpipe}        \\ % UL 17.9 with Muphoten
2022-10-10T04:21	&	59862.1812                    	&	0.6278              	&	$B$     	&	5$\times$60s      	&	-	&	19.7 	&	LOAO-1m     & \cite{2022GCN.32659....1P}   & -             \\ %Ok checked
\hline
2022-10-09T16:21	&	59861.6812                    	&	0.1278              	&	$g^\prime$ 	&	200s       	&	17.66  $\pm$ 0.07  	&	-   	&	GIT        & \cite{2022GCN.32662....1K}    & - \\ %ok checked
2022-10-09T18:21	&	59861.7646                    	&	0.2111              	&	$g^\prime$ 	&	6$\times$60s       	&	18.22  $\pm$ 0.33  	&	-   	&	MeerLICHT      & \cite{2022GCN.32646....1D}  & -       \\ %Ok checked
2022-10-10T05:00	&	59862.2083                    	&	0.6549              	&	$g^\prime$ 	&	300s       	&	18.96  $\pm$ 0.1   	&	-  	&	Nickel-1m   & \cite{2022GCN.32669....1V}       &   -  \\ %ok ckecked
2022-10-10T11:39	&	59862.4854                    	&	0.932               	&	$g^\prime$ 	&	8340s       	&	-	&	18.3  	&	MITSuME   & \cite{2022GCN.32730....1S} & -    \\ %ok checked
2022-10-10T12:25	&	59862.5174                    	&	0.9639              	&	$g^\prime$ 	&	2$\times$150s       	&	-	&	18.3 (3$\sigma$)	&	SLT-40    & \cite{2022GCN.32667....1C} &    -         \\ %ok checked
2022-10-10T16:34	&	59862.6903                    	&	1.1368              	&	$g^\prime$ 	&	2$\times$120s    	&	20.38  $\pm$ 0.19  	&	19.9 ($3\sigma$) 	&	\textcolor{black}{KAO}     & this work & {\sc Muphoten}             \\ %checked upper limit
2022-10-10T16:56	&	59862.7056                    	&	1.1521              	&	$g^\prime$ 	&	600s       	&	20.13  $\pm$ 0.08  	&	-   	&	RTT-150     & \cite{2022GCN.32743....1B}   & -         \\
2022-10-10T17:16	&	59862.7194                    	&	1.166               	&	$g^\prime$ 	&	15$\times$30s     	&	20.53  $\pm$ 0.1   	&	21.0 (3$\sigma$)   	&	AZT-20      & \cite{2022GCN.32769....1B} & -               \\ %checked sarah
2022-10-10T19:40	&	59862.8194                    	&	1.266               	&	$g^\prime$ 	&	3$\times$100s     	&	20.87  $\pm$ 0.36  	&	-   	&	LCOGT     & \cite{2022GCN.32693....1S} & -             \\ %ok checked
2022-10-10T20:17	&	59862.8451                    	&	1.2917              	&	$g^\prime$ 	&	600s       	&	20.44  $\pm$ 0.25  	&	-   	&	RTT-150 & \cite{2022GCN.32743....1B}   & -                \\ %ok checked
2022-10-11T17:10	&	59863.7153                    	&	2.1618              	&	$g^\prime$ 	&	600s       	&	21.15  $\pm$ 0.21  	&	-  	&	RTT-150   &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T02:40	&	59864.1111                    	&	2.5577              	&	$g^\prime$ 	&	-     	&	-	&	23.0   	&	LBTO      &         \cite{2022GCN.32759....1S} & -     \\ %Ale$\times$ please confirm
2022-10-12T03:34	&	59864.1486                    	&	2.5952              	&	$g^\prime$ 	&	3$\times$300s     	&	-	&	22.3  	&	LCOGT     & \cite{2022GCN.32738....1S} &      -       \\ %ok checked
2022-10-15T15:44	&	59867.6556                    	&	6.1021              	&	$g^\prime$ 	&	30$\times$60s     	&	22.6   $\pm$ 0.12  	&	23.4(3$\sigma$)  	&	AZT-20   & \cite{2022GCN.32769....1B} & - \\%ok checked
2022-10-29T05:57	&	59881.2479                    	&	19.6945             	&	$g^\prime$ 	&	3$\times$300s    	&	24.52  $\pm$ 0.2   	&	26.1   	&	\textcolor{black}{CFHT-Megacam}   & this work & \sc{Muphoten} \\
\hline
%2022-10-09T19:36	&	59861.8167                    	&	0.2632              	&	V     	&	e$\times$p       	&	17.48  $\pm$ 0.02  	&	0.0   	&	SCT-0.28  &       \sa{ref}
2022-10-09T13:15:29	&	59861.5524                    	&	-0.0010             	&	$V$  	&	27s     	&	-&	2.0   	&	  \textcolor{black}{Mundrabilla}     & this work     & section~\ref{sec:mundrabilla}      \\
2022-10-09T13:15:59	&	59861.5528                    	&	-0.0007             	&	$V$  	&	27s     	&	-	&	2.0   	&	  \textcolor{black}{Mundrabilla}     & this work     &  section~\ref{sec:mundrabilla}      \\
2022-10-09T13:16:30 & 59861.5531 & -0.0003  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:17:00 & 59861.5535 & 0.0000  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &    section~\ref{sec:mundrabilla}      \\
2022-10-09T13:17:30 & 59861.5538 & 0.0004  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:18:00 & 59861.5542 & 0.0007  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &    section~\ref{sec:mundrabilla}      \\
2022-10-09T13:18:30 & 59861.5545 & 0.0011  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:19:00 & 59861.5549 & 0.0014  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:19:30 & 59861.5552 & 0.0017  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &  section~\ref{sec:mundrabilla}        \\
2022-10-09T13:20:00 & 59861.5556 & 0.0021  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:20:30 & 59861.5559 & 0.0024  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:21:30 & 59861.5566 & 0.0031  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:22:00 & 59861.5569 & 0.0035  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:23:00 & 59861.5576 & 0.0042  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &   section~\ref{sec:mundrabilla}       \\
2022-10-09T13:23:30 & 59861.5580 & 0.0045  & $V$ & 27s    & -  & 3.8 & \textcolor{black}{RawWarRoad}     & this work     &  section~\ref{sec:mundrabilla}        \\
%2022-10-09T19:36	&	59861.8167                    	&	0.2632              	&	$V$     	&	5$\times$180 s      	&	17.46  $\pm$ 0.07  	&	18.6  	&	\textcolor{black}{KNC-SCT-0.28}         & this work  & STDPIPE-force            \\
2022-10-09T19:35:00	&	59861.82118                    	&	0.2677            	&	$V$     	&	5$\times$180s      	&	17.39 $\pm$  0.08  	&  18.3 (5$\sigma$)  	&	\textcolor{black}{KNC-SCT-0.28}         & \cite{2022GCN.32640....1B} \& this work  & \sc{Muphoten}           \\
2022-10-10T04:23	&	59862.1826                    	&	0.6292              	&	$V$     	&	5$\times$60s      	&	18.74  $\pm$ 0.13  	&	19.5 	&	LOAO-1m    &       \cite{2022GCN.32659....1P}     & -    \\
2022-10-10T16:48	&	59862.7                       	&	1.1465              	&	$V$     	&	25$\times$120s   	&	19.36 $\pm$ 0.15	&	19.5   	&	\textcolor{black}{ShAOT60}     & this work  & \sc{STDpipe}            \\
%2022-10-10T19:17	&	59862.8035                    	&	1.25                	&	$V$     	&	11$\times$180 s      	&	-	&	19.1  	&	\textcolor{black}{KNC-SCT-0.28}     & this work    & STDPIPE           \\
2022-10-10T19:16	&	59862.8141                   	&	1.2606               	&	$V$     	&	11$\times$180s      	&	-	&	18.7 (5$\sigma$)  	&	\textcolor{black}{KNC-SCT-0.28}     & this work    &  \sc{Muphoten} \\ %UL 19.3 Damien stdpipe
2022-10-14T20:13	&	59866.8768                   	&	5.3233          	&	$V$     	&	180$\times$32s      	&	21.55   $\pm$ 0.24  	&	21.2 (5$\sigma$) 	&	\textcolor{black}{KNC-T-CAT}     & this work & \sc{STDpipe}       \\ %checked ?
\hline
2022-10-09T19:51	&	59861.8271                    	&	0.2736              	&	$R_c$  	&	5$\times$180s       	&	16.26   $\pm$ 0.05  	&  17.9 (5$\sigma$) &	\textcolor{black}{KNC-SCT-0.28}     & \cite{2022GCN.32640....1B} \& this work   & \sc{Muphoten}             \\ %Broens 16.6 Damien 16.59 UL 18.8
%2022-10-09T19:51	&	59861.8271                    	&	0.2736              	&	\sa{$R_c$} 	&	5$\times$180 s      	&	16.59  $\pm$ 0.03  	&	18.8  &		\textcolor{black}{KNC-SCT-0.28}     & \cite{2022GCN.32640....1B} \& this work   & calib. ps1/r               \\ %okchecked
2022-10-10T11:39	&	59862.4854                    	&	0.932               	&	$R_c$  	&	60s        	&	-	&	17.0  	&	MITSuME   & \cite{2022GCN.32730....1S} & -            \\
2022-10-10T14:56	&	59862.6347                    	&	1.0813              	&	$R_c$  	&	6$\times$180s    	&	18.21  $\pm$ 0.14  	&	18.5 	&	\textcolor{black}{UBAI-ST60}    & this work  & \sc{Muphoten}           \\
2022-10-10T15:53	&	59862.6774                    	&	1.124               	&	$R_c$  	&	15$\times$90s    	&	-	&	-   	&	\textcolor{black}{ShAOT60}      & this work   & VETO           \\
2022-10-10T18:32	&	59862.7809                    	&	1.2274              	&	$R_c$  	&	25$\times$30s    	&	18.1   $\pm$ 0.08  	&	19.3 	&	\textcolor{black}{Lisnyky-AZT-8}     & this work  & \sc{Muphoten}             \\
2022-10-10T18:45	&	59862.7899                    	&	1.2365              	&	$R_c$  	&	25$\times$30s    	&	18.24  $\pm$ 0.08  	&	19.1 	&	\textcolor{black}{Lisnyky-AZT-8}    & this work & \sc{Muphoten}  \\
2022-10-10T19:43:14	&	59862.8290                   	&	1.2755              	&	$R_c$ 	&	 7$\times$180s    	&	-  	&	18.2 (5$\sigma$)  &	\textcolor{black}{KNC-SCT-0.28}     & this work   & \sc{Muphoten}               \\ %okchecked Damien 18.44+-0.13 UL19.0
2022-10-11T19:52:44	&	59863.8292                    	&	2.2956              	&	$R_c$ 	&	20$\times$180s      	&	-	&	18.8 (5$\sigma$) 	&	\textcolor{black}{KNC-SCT-0.28}     & \cite{2022GCN.32640....1B} \& this work   & \sc{Muphoten}    \\ %okchecked this one is weird Damien UL 19.8
2022-10-11T18:44	&	59863.8576                    	&	2.3042              	&	$R_c$  	&	111$\times$60s   	&	19.22  $\pm$ 0.08  	&	20.5 	&	\textcolor{black}{Lisnyky-AZT-8}      & this work & \sc{Muphoten}             \\
2022-10-12T14:24	&	59864.6139                    	&	3.0604              	&	$R_c$  	&	5$\times$240s    	&	-  	&	- 	&	\textcolor{black}{UBAI-ST60}    & this work & VETO             \\
2022-10-12T19:40	&	59864.8403                    	&	3.2868              	&	$R_c$  	&	30$\times$60s    	&	19.98  $\pm$ 0.11  	&	20.1 	&	\textcolor{black}{Lisnyky-AZT-8}      & this work  & \sc{Muphoten}            \\
2022-10-14T14:10	&	59866.6208                    	&	5.0674              	&	$R_c$  	&	11$\times$240s   	&	-	&	18.5 	&	\textcolor{black}{UBAI-ST60}       & this work    & \sc{Muphoten}       \\
2022-10-21T22:58	&	59874.0102                    	&	12.4567             	&	$R_c$ 	&	460$\times$10s   	&	-	&	19.9 	&	\textcolor{black}{VIRT}          & this work & \sc{Muphoten} \\
2022-10-22T03:34:20	&	59874.1697                    	&	12.6162             	&	$R_c$ 	&	6$\times$600 s     	&	-	&	19.4 (5$\sigma$) 	&	\textcolor{black}{KNC-iT11}     & this work & \sc{STDpipe}          \\
\hline
2022-10-09T14:25	&	59861.6007                    	&	0.0472              	&	$r^\prime$ 	&	-       	&	14.93  $\pm$ 0.1   	&	-   	&	NEXT          &  \cite{2022GCN.32647....1X} & -             \\ %ok checked
2022-10-09T14:27	&	59861.6021                    	&	0.0486              	&	$r^\prime$ 	&	120s      	&	14.84  $\pm$ 0.09  	&	20.8  	&	Mondy     & \cite{2022GCN.32645....1B} & -              \\
2022-10-09T15:36	&	59861.6507                    	&	0.0972              	&	$r^\prime$ 	&	180s    	&	15.92  $\pm$ 0.12  	&	16.5   	&	\textcolor{black}{TRE}        & this work  & \sc{STDpipe} \& \sc{Muphoten}           \\
2022-10-09T15:39	&	59861.6528                    	&	0.0993              	&	$r^\prime$ 	&	180s    	&	15.82  $\pm$ 0.18  	&	16.7   	&	\textcolor{black}{TRE}      & this work     & \sc{STDpipe} \& \sc{Muphoten}             \\
2022-10-09T15:40	&	59861.6530                    	&	0.0995              	&	$r^\prime$ 	&	180s    	&	15.74  $\pm$ 0.28  	&	16.1   	&	\textcolor{black}{TRE}       & this work     & \sc{STDpipe} \& \sc{Muphoten}            \\
2022-10-09T16:25	&	59861.684                     	&	0.1306              	&	$r^\prime$ 	&	200s       	&	16.16  $\pm$ 0.07  	&	-   	&	GIT            & \cite{2022GCN.32662....1K}   & -         \\
%ok checked
2022-10-09T17:28	&	59861.7283                    	&	0.1748               	&	$r^\prime$ 	&	180s    	&	16.4  $\pm$ 0.3  	&	16.3   	&	\textcolor{black}{TRE}     & this work       & \sc{STDpipe} \& \sc{Muphoten}            \\
2022-10-09T17:29	&	59861.7285                    	&	0.1750               	&	$r^\prime$ 	&	180s    	&	15.88  $\pm$ 0.23  	&	16.3   	&	\textcolor{black}{TRE}     & this work       & \sc{STDpipe} \& \sc{Muphoten}           \\
2022-10-09T18:25	&	59861.7674                    	&	0.2139              	&	$r^\prime$ 	&	-       	&	16.5   $\pm$ 0.1   	&	-   	&	NEXT      &  \cite{2022GCN.32647....1X} & -             \\
%ok checked
2022-10-09T18:23	&	59861.766                     	&	0.2125              	&	$r^\prime$ 	&	6$\times$60s       	&	16.76  $\pm$ 0.08  	&	-   	&	MeerLICHT    &   \cite{2022GCN.32944....1D} &      -       \\ %ok checked
%	&	                    	&	            	&		&	       	&	  	&	   	&	    &   \cite{2022GCN.32944....1D} &             \\ %ok checked
2022-10-09T18:49	&	59861.784                     	&	0.2306              	&	$r^\prime$  	&	90s       	&	16.57  $\pm$ 0.02  	&	-   	&	OSN-0.9   & \cite{2022GCN.32644....1H} &     -           \\
2022-10-09T23:58	&	59861.9986                    	&	0.4452              	&	$r^\prime$ 	&	-       	&	17.36  $\pm$ 0.12  	&	-   	&	REM          & \cite{2022GCN.32652....1B}   & -         \\
2022-10-10T04:25	&	59862.184                     	&	0.6306              	&	$r^\prime$  	&	60$\times$5s      	&	17.55  $\pm$ 0.06  	&	19.8 	&	LOAO-1m    &       \cite{2022GCN.32659....1P}     & -    \\
2022-10-10T05:00	&	59862.2083                    	&	0.6549              	&	$r^\prime$ 	&	300s       	&	17.8   $\pm$ 0.1   	&	-   	&	Nickel-1m     & \cite{2022GCN.32669....1V}       &   -  \\ %ok ckecked
 %ok checked
\hline
\end{tabular}}
\end{table*}

\begin{table*}
\addtocounter{table}{-1}
\caption{Continued.}
\scalebox{0.6}{
\begin{tabular}{|l|cc|c|l|l|l|c|c|c|}
2022-10-10T12:25	&	59862.5174                    	&	0.9639              	&	$r^\prime$ 	&	2$\times$150s       	&	18.67  $\pm$ 0.16  	&	-   	&	SLT-40      & \cite{2022GCN.32667....1C} &    -         \\
2022-10-10T16:33	&	59862.7023                    	&	1.1489              	&	$r^\prime$ 	&	11$\times$100s   	&	18.65  $\pm$ 0.08  	&	20.9  	&	KAO   & this work  &  \sc{Muphoten} \\
2022-10-10T17:06	&	59862.7125                    	&	1.159               	&	$r^\prime$ 	&	600s       	&	18.65  $\pm$ 0.02  	&	-   	&	RTT-150     & \cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-10T17:14	&	59862.7181                    	&	1.1646              	&	$r^\prime$ 	&	18$\times$30s     	&	18.64  $\pm$ 0.03  	&	20.8 (3$\sigma$)   	&	AZT-20       &  \cite{2022GCN.32670....1K} & -               \\ %ok checked
2022-10-10T19:26	&	59862.8097                    	&	1.2563              	&	$r^\prime$	&	2$\times$300s      	&	18.74  $\pm$ 0.12  	&	-   	&	RC-80         &  \cite{2022GCN.32709....1V} &   -          \\ % ok checked
2022-10-10T19:40	&	59862.8194                    	&	1.266               	&	$r^\prime$ 	&	3$\times$100s     	&	18.8   $\pm$ 0.21  	&	-   	&	LCOGT     & \cite{2022GCN.32693....1S} & -              \\ %ok checked
2022-10-10T20:30	&	59862.8611                    	&	1.3077              	&	$r^\prime$ 	&	2$\times$300s    	&	18.86   $\pm$ 0.04   	&	20.5 	&	\textcolor{black}{C2PU/Omicron}    & this work  & \sc{STDpipe} \& \sc{Muphoten}         \\
2022-10-10T20:50	&	59862.8681                    	&	1.3146              	&	$r^\prime$ 	&	600s       	&	18.81  $\pm$ 0.05  	&	-   	&	RTT-150      & \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-11T00:15	&	59863.0444                  	&	1.4909              	&	$r^\prime$ 	&	16$\times$360s      	&	18.89  $\pm$ 0.06   	&	20.4 (5$\sigma$)	&	\textcolor{black}{KNC-C14/Ste-Sophie}   & this work  & \sc{STDpipe}    \\
2022-10-11T00:58	&	59863.0846                    	&	1.5312              	&	$r^\prime$	&	  59$\times$120s    	&	18.93  $\pm$ 0.09  	&	19.8 (5$\sigma$)  &	\textcolor{black}{KNC-C11-FREE}     & this work  & \sc{STDpipe}              \\
2022-10-11T16:37	&	59863.6924                    	&	2.1389              	&	$r^\prime$ 	&	600s       	&	19.53  $\pm$ 0.04  	&	-   	&	RTT-150   &   \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-11T20:41	&	59863.8617                  	&	2.3083              	&	$r^\prime$ 	&	-      	&	19.36  $\pm$ 0.15  	&	19.8 (5$\sigma$) 	&	\textcolor{black}{KNC-Parent}    & this work  & \sc{STDPipe}             \\
2022-10-11T20:44	&	59863.8639                    	&	2.3104              	&	$r^\prime$ 	&	600s       	&	19.67  $\pm$ 0.11  	&	-   	&	RTT-150  &   \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-12T01:36	&	59864.1041                    	&	2.5506             	&	$r^\prime$ 	&	31$\times$180s      	&	19.56  $\pm$ 0.12  	&	20.2 (5$\sigma$) 	&	\textcolor{black}{KNC-LCO/McDO-0.4m}     & this work  & \sc{STDpipe}            \\
2022-10-12T03:34	&	59864.1486                    	&	2.5952              	&	$r^\prime$	&	3$\times$300s     	&	-	&	21.4  	&	LCOGT       & \cite{2022GCN.32738....1S} &      -        \\ %ok checked
2022-10-12T17:05	&	59864.7118                    	&	3.1583              	&	$r^\prime$ 	&	600s       	&	20.03 $\pm$ 0.06  	&	-   	&	RTT-150  & \cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T17:38	&	59864.7347                    	&	3.1813              	&	$r^\prime$ 	&	600s       	&	19.97  $\pm$ 0.08  	&	-   	&	RTT-150  & \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-12T18:10	&	59864.7569                    	&	3.2035              	&	$r^\prime$ 	&	600s       	&	20.07  $\pm$ 0.19  	&	-   	&	RTT-150    & \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-12T18:42	&	59864.7792                    	&	3.2257              	&	$r^\prime$ 	&	600s       	&	20.32  $\pm$ 0.17  	&	-   	&	RTT-150     & \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-12T19:15	&	59864.8409                    	&	3.2874              	&	$r^\prime$ 	&	30$\times$120s      	&	-	&	18.4  	&	KNC-C11-ATLAS     & this work   &   \sc{STDPipe}       \\
2022-10-12T19:46	&	59864.8236                    	&	3.2702              	&	$r^\prime$ 	&	600s      	&	20.17  $\pm$ 0.12  	&	-  	&	RTT-150    & \cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T19:40	&	59864.8194                    	&	3.266               	&	$r^\prime$ 	&	1800s     	&	20.23  $\pm$ 0.09  	&	-   	&	OHP       &  \cite{2022GCN.32753....1S} & -        \\ % checked damien
%2022-10-12T19:40	&	59864.8194                    	&	3.266               	&	sdssr 	&	2$\times$600 s     	&	20.23  $\pm$ 0.09  	&	0.0   	&	OHP       &  \cite{2022GCN.32753....1S} & STDPIPE-force          \\ % checked damien
2022-10-12T20:18	&	59864.8458                    	&	3.2924              	&	$r^\prime$ 	&	300s       	&	20.58  $\pm$ 0.7   	&	-   	&	RC-80         &  \cite{2022GCN.32709....1V} &   -          \\ % ok checked
2022-10-12T20:25	&	59864.8507                    	&	3.2972              	&	$r^\prime$ 	&	600s       	&	20.26  $\pm$ 0.16  	&	-   	&	RTT-150        & \cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T20:57	&	59864.8729                    	&	3.3195              	&	$r^\prime$ 	&	600s       	&	20.24  $\pm$ 0.19  	&	-   	&	RTT-150         & \cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-13T03:09	&	59865.1312                    	&	3.5778              	&	$r^\prime$ 	&	-       	&	20.44  $\pm$ 0.05  	&	-   	& LDT & \cite{2022GCN.32739....1O} &    -               \\ %ok checked
2022-10-13T17:37	&	59865.7632                    	&	4.2097              	&	$r^\prime$ 	&	21$\times$120s   	&	-	&	20.2  	&	KAO   & this work  & \sc{Muphoten}                  \\
2022-10-13T16:53	&	59865.7035                    	&	4.15                	&	$r^\prime$	&	600s       	&	20.53  $\pm$ 0.09  	&	-  	&	RTT-150         &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T17:25	&	59865.7257                    	&	4.1722              	&	$r^\prime$ 	&	600s       	&	20.63  $\pm$ 0.09  	&	-   	&	RTT-150         &  \cite{2022GCN.32752....1B} & -              \\ %ok checked
2022-10-13T17:58	&	59865.7486                    	&	4.1952              	&	$r^\prime$ 	&	600s       	&	20.71  $\pm$ 0.15  	&	-   	&	RTT-150         &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T18:30	&	59865.7708                    	&	4.2174              	&	$r^\prime$ 	&	600s       	&	20.54  $\pm$ 0.1   	&	-   	&	RTT-150          &  \cite{2022GCN.32752....1B} & -              \\ %ok checked
2022-10-13T19:02	&	59865.7931                    	&	4.2396              	&	$r^\prime$ 	&	600s       	&	20.55  $\pm$ 0.12  	&	-   	&	RTT-150         &  \cite{2022GCN.32752....1B} & -             \\ %ok checked
2022-10-13T19:35	&	59865.816                     	&	4.2625              	&	$r^\prime$ 	&	600s       	&	20.74  $\pm$ 0.16  	&	-   	&	RTT-150       &  \cite{2022GCN.32752....1B} & -              \\ %ok checked
2022-10-13T20:08	&	59865.8389                    	&	4.2854              	&	$r^\prime$ 	&	600s       	&	20.9   $\pm$ 0.23  	&	-   	&	RTT-150       &  \cite{2022GCN.32752....1B} & -              \\ %ok checked
2022-10-13T20:43	&	59865.8632                    	&	4.3097              	&	$r^\prime$ 	&	600s       	&	20.86  $\pm$ 0.27  	&	-   	&	RTT-150         &  \cite{2022GCN.32752....1B} & -              \\ %ok checked
2022-10-14T05:27	&	59866.2271                    	&	4.6736              	&	$r^\prime$ 	&	-      	&	20.92  $\pm$ 0.05  	 & -    	&	Pan-STARRS     & \cite{2022GCN.32758....1H} & -           \\
2022-10-15T14:40	&	59867.6111                    	&	6.0577              	&	$r^\prime$ 	&	30$\times$60s     	&	20.96  $\pm$ 0.05  	&	22.9 (3$\sigma$)  	&	AZT-20           & \cite{2022GCN.32769....1B} & - \\%ok checked
2022-10-15T06:34	&	59867.2736                    	&	5.7202              	&	$r^\prime$ 	&	-       	&	21.13  $\pm$ 0.06  	&	-   	&	Faulkes     & \cite{2022GCN.32771....1S} & -               \\ % ok checked
2022-10-16T14:41	&	59868.6118                    	&	7.0583              	&	$r^\prime$ 	&	200$\times$25s       	&	21.3   $\pm$ 0.04  	&	-   	&	DFOT            & \cite{2022GCN.32811....1G} & -           \\
2022-10-19T02:05	&	59871.0868                    	&	9.5333              	&	$r^\prime$ 	&	-       	&	21.68  $\pm$ 0.07  	&	-   	&	LDT              &  \cite{2022GCN.32799....1O}  &  -        \\
%2022-10-19T18:26	&	59871.8201                    	&	10.2667             	&	$r^\prime$ 	&	15$\times$300 s   	&	21.76  $\pm$ 0.18  	&	21.91 	&	\textcolor{black}{C2PU/Omicron}   & this work   &   MUPHOTEN-detec      \\
2022-10-19T18:26	&	59871.8201                    	&	10.2667             	&	$r^\prime$ 	&	4$\times$300s   	&	21.8  $\pm$ 0.07  	&	21.9 	&	C2PU/Omicron   & this work   &   \sc{STDpipe} \& \sc{Muphoten}     \\
%2022-10-19T19:33:38.265,59871.81502621528, 10.262 C2PU-Omicron,sdssr,21.8,0.07,0.0,4$\times$300 s,AB,ps1,rmag STDPIPE, calib. ps1/r
2022-10-20T16:11	&	59872.6847                    	&	11.1313             	&	$r^\prime$  	&	3$\times$300s    	&	21.86  $\pm$ 0.18  	&	21.8  	&	UBAI-AZT22    & this work    & \sc{Muphoten}        \\
2022-10-21T14:33	&	59873.6062                    	&	12.0528             	&	$r^\prime$ 	&	30$\times$60s     	&	21.94  $\pm$ 0.07  	&	23.9(3$\sigma$)  	&	AZT-20             & \cite{2022GCN.32818....1B}  &  -       \\
2022-10-23T00:59:10	&	59875.0757                    	&	13.5222             	&	$r^\prime$ 	&	31$\times$180s      	&	-	&	19.4  (5$\sigma$)	&	KNC-C11-FREE     & this work  & \sc{STDpipe}         \\
2022-10-25T01:59:52	&	59877.1045                   	&	15.5510            	&		$r^\prime$  	&	6$\times$600s     	&	-	&	20.5 (5$\sigma$) 	& KNC-iT11    & this work   & \sc{STDpipe}         \\
2022-10-27T00:45:41	&	59879.0501                      	&	17.4967             	&	$r^\prime$	& 26$\times$120s     	&	-	&	20.0  (5$\sigma$)	&	KNC-C11-FREE    & this work  & \sc{STDpipe}          \\
2022-10-29T05:50	&	59881.25                      	&	19.6965             	&	$r^\prime$ 	&	2$\times$300s    	&	22.69   $\pm$ 0.05   	&	25.5   	&	\textcolor{black}{CFHT-Megacam}     & this work & \sc{STDpipe} \& \sc{Muphoten}        \\
\hline
%\multicolumn{10}{c}{$i^\prime$-band} \\
2022-10-09T18:26:56	&	59861.7687     	&	0.2152             	&	$i^\prime$ 	&	6$\times$60s      	&	15.58  $\pm$ 0.03  	&	-  	&	MeerLICHT      & \cite{2022GCN.32646....1D}  & -             \\
2022-10-10T02:04:32	&	59862.0868                   	&	0.5333              	&	$i^\prime$ 	&	300s      	&	16.24  $\pm$ 0.05  	&	17.9 (5$\sigma$)  	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}           \\ %ok checked
2022-10-10T02:10:06	&	59862.0907                    	&	0.5372              	&	$i^\prime$ 	&	300s      	&	16.25  $\pm$ 0.05  	&	17.9 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T02:15:41 &	59862.0945                   	&	0.5411              	&	$i^\prime$ 	&	300s      	&	16.28  $\pm$ 0.05  	&	17.9 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T02:21:15	&	59862.0984                    	&	0.5450              	&	$i^\prime$ 	&	300s      	&	16.34  $\pm$ 0.05  	&	17.9 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}           \\ %ok checked
2022-10-10T02:26:50	&	59862.1023                   	&	0.5489             	&	$i^\prime$ 	&	300s      	&	16.38  $\pm$ 0.06  	&	17.8 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}           \\ %ok checked
2022-10-10T02:32:25 &	59862.1062                    	&	0.5527              	&	$i^\prime$ 	&	300s      	&	16.37  $\pm$ 0.05  	&	17.9 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}          \\ %ok checked
2022-10-10T02:38:55	&	59862.1107                   	&	0.5572              	&	$i^\prime$ 	&	300s      	&	16.46  $\pm$ 0.05  	&	18.0 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T02:44:29	&	59862.1107                    	&	0.5611              	&	$i^\prime$ 	&	300s      	&	16.44  $\pm$ 0.05  	&	17.9 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T02:50:04 &	59862.1184                    	&	0.5650              	&	$i^\prime$ 	&	300s      	&	16.41  $\pm$ 0.06  	&	17.9 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T02:55:39	&	59862.1223                    	&	0.5689              	&	$i^\prime$ 	&	300s      	&	16.27  $\pm$ 0.05  	&	17.8 (5$\sigma$)	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T03:01:14	&	59862.1262                    	&	0.5727              	&	$i^\prime$ 	&	300s      	&	16.44  $\pm$ 0.06  	&	17.8 (5$\sigma$) 	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T03:06:48	&	59862.1301                    	&	0.5766              	&	$i^\prime$ 	&	300s      	&	16.58  $\pm$ 0.07  	&	17.8 (5$\sigma$)	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\ %ok checked
2022-10-10T04:26	&	59862.1847                    	&	0.6313              	&	$i^\prime$     	&	60$\times$5s      	&	16.41  $\pm$ 0.05  	&	19.56 	&	LOAO-1m &   \cite{2022GCN.32659....1P}     & -    \\
2022-10-10T12:25	&	59862.5174                    	&	0.9639              	&	$i^\prime$ 	&	2$\times$150s       	&	17.38  $\pm$ 0.09  	&	-   	&	SLT-40           & \cite{2022GCN.32667....1C} &    -       \\ %ok checked
2022-10-10T16:59	&	59862.716                     	&	1.1625              	&	$i^\prime$ 	&	9$\times$80s     	&	17.67  $\pm$ 0.05  	&	20.7  	&	\textcolor{black}{KAO}       & this work  & \sc{Muphoten}                \\
2022-10-10T17:23	&	59862.7243                    	&	1.1708              	&	$i^\prime$ 	&	15$\times$30s     	&	17.58  $\pm$ 0.01  	& 20.7 (3$\sigma$)   	&	AZT-20      & \cite{2022GCN.32769....1B} & -              \\ %checked sarah
2022-10-10T17:17	&	59862.7201                    	&	1.1667              	&	$i^\prime$ 	&	600s       	&	17.52  $\pm$ 0.01  	&	-   	&	RTT-150         & \cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-10T18:20:07	&	59862.7938                    	&	1.2255              	&	$i^\prime$ 	&	14$\times$180s      	&	17.47  $\pm$ 0.09  	&	17.6 (5$\sigma$)  	&	\textcolor{black}{KNC-IRIS}    & this work  & \sc{STDpipe}    \\
2022-10-10T19:26	&	59862.8097                    	&	1.2563              	&	$i^\prime$	&	2$\times$300s       	&	17.5   $\pm$ 0.12  	&	-   	&	RC-80            &  \cite{2022GCN.32709....1V} &   -          \\ % ok checked
2022-10-10T21:01	&	59862.8757                    	&	1.3222              	&	$i^\prime$ 	&	600s       	&	17.69  $\pm$ 0.02  	&	-   	&	RTT-150           & \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-11T06:07:28	&	59863.2569                    	&	1.7035              	&	$i^\prime$ 	&	300s      	&	17.85  $\pm$ 0.13  	&	18.1 (5$\sigma$) 	&	\textcolor{black}{KNC-iT24}     & this work  & \sc{STDpipe}              \\
2022-10-11T06:12:57	&	59863.2607                   	&	1.7072              	&	$i^\prime$ 	& 300s      	&	18.24  $\pm$ 0.22  	&	18.2 (5$\sigma$)  	&	\textcolor{black}{KNC-iT24}     & this work  & \sc{STDpipe}              \\
2022-10-11T00:54	&	59863.0375                    	&	1.484               	&	$i^\prime$ 	&	-       	&	17.92  $\pm$ 0.06  	&	-   	&	BlackGEM          & \cite{2022GCN.32678....1G} & -         \\
2022-10-11T16:48	&	59863.7                       	&	2.1465              	&	$i^\prime$ 	&	600s       	&	18.4   $\pm$ 0.02  	&	-   	&	RTT-150          & \cite{2022GCN.32743....1B}   & -              \\ % ok checked
2022-10-11T18:46:47	&	59863.8193                    	&	2.2659              	&	$i^\prime$ 	&	199$\times$32s      	&	18.64  $\pm$ 0.21  	&	18.7 (5$\sigma$) 	&	\textcolor{black}{KNC-EHEA-200F5}     & this work & \sc{STDpipe}          \\ %ok checked
2022-10-11T20:56	&	59863.8722                    	&	2.3188              	&	$i^\prime$ 	&	600s       	&	18.49  $\pm$ 0.04  	&	-   	&	RTT-150          & \cite{2022GCN.32743....1B}   & -              \\ % ok checked
 %ok checked}	&	\DT{59862.1301}                    	&	\DT{0.5766}              	&	\DT{$i^\prime$} 	&	1$\times$60s      	&	16.58  $\pm$ 0.07  	&	17.8 	&	\textcolor{black}{KNC-BGO}     & this work    & STDPIPE, calib. ps1/i           \\ %ok checked
2022-10-12T00:58:02	&	59864.0626                    	&	2.5092              	&	$i^\prime$ 	&	$11\times300$s      	&	18.44  $\pm$ 0.09  	&	19.0 (5$\sigma$)	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}            \\
2022-10-12T02:07:18	&	59864.1083                    	&	2.5548              	&	$i^\prime$ 	&	11$\times$300s      	&	18.74  $\pm$ 0.13  	&	19.3 (5$\sigma$) 	&	\textcolor{black}{KNC-C11-FREE}   & this work   & \sc{STDpipe}            \\ %ok checkeck           \\
2022-10-12T02:40	&	59864.1111                    	&	2.5577              	&	$i^\prime$ 	&	-       	&	19.0   $\pm$ 0.2   	&	-   	&	LBTO          & \cite{2022GCN.32759....1S} & - \\ %ale$\times$ please confirm
2022-10-12T03:34	&	59864.1486                    	&	2.5952              	&	$i^\prime$ 	&	3$\times$300s     	&	-	&	20.5  	&	LCOGT     & \cite{2022GCN.32738....1S} &       -        \\ %ok checked                \\
2022-10-12T16:54	&	59864.7042                    	&	3.1507              	&	$i^\prime$ 	&	600s       	&	18.82  $\pm$ 0.03  	&	-   	&	RTT-150           &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T17:27	&	59864.7271                    	&	3.1736              	&	$i^\prime$ 	&	600s       	&	19.02  $\pm$ 0.07  	&	-   	&	RTT-150             &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T17:59	&	59864.7493                    	&	3.1958              	&	$i^\prime$ 	&	600s       	&	19.09  $\pm$ 0.1   	&	-   	&	RTT-150           &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T18:31	&	59864.7715                    	&	3.2181              	&	$i^\prime$ 	&	600s      	&	18.95  $\pm$ 0.07  	&	-   	&	RTT-150           &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T19:03	&	59864.7938                    	&	3.2403              	&	$i^\prime$ 	&	600s       	&	18.93  $\pm$ 0.04  	&	-   	&	RTT-150            &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T19:36	&	59864.8167                    	&	3.2632              	&	$i^\prime$ 	&	600s       	&	18.93  $\pm$ 0.04  	&	-   	&	RTT-150            &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T19:40	&	59864.8194                    	&	3.266               	&	$i^\prime$ 	&	3$\times$600s     	&	18.91  $\pm$ 0.11  	&	-  	&	OHP             &  \cite{2022GCN.32753....1S} & -         \\ % checked damien
2022-10-12T20:08	&	59864.8389                    	&	3.2854              	&	$i^\prime$ 	&	600s       	&	18.92  $\pm$ 0.04  	&	-   	&	RTT-150          &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T20:18	&	59864.8458                    	&	3.2924              	&	$i^\prime$ 	&	300s       	&	18.74  $\pm$ 0.18  	&	-   	&	RC-80              &  \cite{2022GCN.32709....1V} &   -          \\ % ok checked
\end{tabular}}
\end{table*}

\begin{table*}
\addtocounter{table}{-1}
\caption{Continued.}
\scalebox{0.6}{
\begin{tabular}{|l|cc|c|l|l|l|c|c|c|}
2022-10-13T02:36:45	&	59865.1069                    	&	3.5534              	&	$i^\prime$ 	&	$12\times300$s      	&	19.50  $\pm$ 0.22  	&	19.4 (5$\sigma$)	&	\textcolor{black}{KNC-BGO}     & this work    & \sc{STDpipe}     \\
2022-10-13T02:24:22	&	59865.1149                       	&	3.5614              	&	$i^\prime$ 	&	20$\times$120s      	&	-  	&	18.7 (5$\sigma$)  	&	\textcolor{black}{KNC-iT11}       & this work & \sc{STDpipe}                \\
2022-10-13T03:09	&	59865.1312                    	&	3.5778              	&	$i^\prime$ 	&	-      	&	19.37  $\pm$ 0.05  	&	-   	&	LDT       & \cite{2022GCN.32739....1O} &    -               \\ %ok checked
2022-10-13T17:04	&	59865.7111                    	&	4.1577              	&	$i^\prime$ 	&	600s       	&	19.51  $\pm$ 0.06  	&	-   	&	RTT-150          &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T17:36	&	59865.7333                    	&	4.1799              	&	$i^\prime$ 	&	600s       	&	19.41  $\pm$ 0.05  	&	-   	&	RTT-150           &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T18:09	&	59865.7562                    	&	4.2028              	&	$i^\prime$ 	&	600s       	&	19.52  $\pm$ 0.05  	&	-   	&	RTT-150           &  \cite{2022GCN.32752....1B} & -              \\ %ok checked\
2022-10-13T17:42	&	59865.7642                    	&	4.2108              	&	$i^\prime$ 	&	21$\times$110s   	&	19.73  $\pm$ 0.3   	&	20.3  	&	\textcolor{black}{KAO}     & this work & \sc{Muphoten}                 \\
2022-10-13T18:41	&	59865.7785                    	&	4.225               	&	$i^\prime$ 	&	600s       	&	19.44  $\pm$ 0.04  	&	-   	&	RTT-150           &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T19:13	&	59865.8007                    	&	4.2472              	&	$i^\prime$	    &	600s       	&	19.45  $\pm$ 0.05  	&	-   	&	RTT-150            &  \cite{2022GCN.32752....1B} & -               \\ %ok checked\
2022-10-13T19:46	&	59865.8236                    	&	4.2702              	&	$i^\prime$ 	&	600s       	&	19.43  $\pm$ 0.05  	&	-   	&	RTT-150          &  \cite{2022GCN.32752....1B} & -               \\ %ok checked\
2022-10-13T20:18	&	59865.8458                    	&	4.2924              	&	$i^\prime$ 	&	600s       	&	19.48  $\pm$ 0.06  	&	-   	&	RTT-150          &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T20:53	&	59865.8701                    	&	4.3167              	&	$i^\prime$ 	&	600s       	&	19.5   $\pm$ 0.07  	&	-   	&	RTT-150           &  \cite{2022GCN.32752....1B} & -               \\ %ok checked\
2022-10-14T00:04	&	59866.0028                    	&	4.4493              	&	$i^\prime$ 	&	-       	&	19.89  $\pm$ 0.05  	&	-   	&	VLT               &  \cite{2022GCN.32765....1I} &   -               \\ %ok checked\
2022-10-14T00:40	&	59866.0278                    	&	4.4743              	&	$i^\prime$ 	&	7$\times$60s      	&	19.8   $\pm$ 0.5   	&	-   	&	GMOS             &  \cite{2022GCN.32749....1R} &     -      \\ %ok checked
2022-10-15T06:34	&	59867.2736                    	&	5.7202              	&	$i^\prime$ 	&	-       	&	20.01  $\pm$ 0.05  	&	-   	&	Faulkes     & \cite{2022GCN.32771....1S} & -               \\ %ok checked
2022-10-15T14:11	&	59867.591                     	&	6.0375              	&	$i^\prime$ 	&	30$\times$60s     	&	20.0   $\pm$ 0.04  	&	23.2 (3$\sigma$)  	&	AZT-20          & \cite{2022GCN.32769....1B} &  - \\%ok checked
2022-10-19T02:05	&	59871.0868                    	&	9.5333              	&	$i^\prime$	&	-       	&	20.72  $\pm$ 0.05  	&	-  	&	LDT              &  \cite{2022GCN.32799....1O}  &  -       \\
2022-10-21T15:04	&	59873.6278                    	&	12.0743             	&	$i^\prime$ 	&	30$\times$60s     	&	20.72  $\pm$ 0.11  	&	23.3(3$\sigma$)  	&	AZT-20             & \cite{2022GCN.32818....1B}  &  -       \\
2022-10-29T06:09	&	59881.2632                    	&	19.7097             	&	$i^\prime$ 	&	2$\times$300s    	&	21.87  $\pm$ 0.05  	&	24.5  	&	\textcolor{black}{CFHT-Megacam}     & this work   & \sc{STDpipe}  \& \sc{Muphoten}       \\ %ok checked
\hline
%\multicolumn{10}{c}{$I_c$-band} \\
%\hline
2022-10-09T20:05:19	&	59861.8422                    	&	0.2887               	&	$I_c$ 	&	5$\times$180s      	&	15.21  $\pm$ 0.04  	&	17.0 (5$\sigma$)  	&		\textcolor{black}{KNC-SCT-0.28}      & this work   & \sc{Muphoten}         \\ %ok checke Damien 15.65+-0.3 UL 18
2022-10-10T05:00	&	59862.2083                    	&	0.6549              	&	$I_c$ 	&	300s       	&	16.74  $\pm$ 0.1   	&	-   	&	Nickel-1m  &       \cite{2022GCN.32669....1V}       &   -  \\ %ok ckecked
%2022-10-09T20:06	&	59861.8375                    	&	0.284               	&	$I_c$     	&	\sa{-}       	&	15.76  $\pm$ 0.06  	&	-   	&	\textcolor{black}{KNC-SCT-0.28}   & \cite{2022GCN.32640....1B} \& this work   & APASS DR9             \\ % Damien tu peu$\times$ refaire l'analyse stp ?
2022-10-10T11:39	&	59862.4854                    	&	0.932               	&	$I_c$     	&	8340s        	&	17.1   $\pm$ 0.2   	&	-   	&	MITSuME      & \cite{2022GCN.32730....1S} & - \\ % ok checked
2022-10-10T20:04:25	&	59862.8436                    	&	1.2902              	&	$I_c$ 	&	7$\times$180s      	&	17.12   $\pm$ 0.13  	&	17.0 (5$\sigma$)  	&	\textcolor{black}{KNC-SCT-0.28}      & this work   & \sc{Muphoten}          \\ %ok checked Damien 17.6+-0.13 UL 18.1
2022-10-11T18:14	&	59863.7958                    	&	2.2424              	&	$I_c$     	&	52$\times$60s    	&	-	&	-  	&	\textcolor{black}{AbAO-T70}   & this work  & VETO        \\
2022-10-11T21:06:16	&	59863.9043                    	&	2.3509              	& 	$I_c$ 	&	24$\times$180s      	&	-   	&	17.6 (5$\sigma$) 	& \textcolor{black}{KNC-SCT-0.28}      & this work   & \sc{Muphoten}         \\ %ok checked Damien 18.8+-0.2 UL 18.9
2022-10-12T18:11	&	59864.7889                    	&	3.2354              	&	$I_c$     	&	45$\times$60s    	&	-  	&	- 	&	\textcolor{black}{Lisnyky-AZT-8}     & this work  &  VETO     \\
%2022-10-12T18:11	&	59864.7889                    	&	3.2354              	&	$I_c$     	&	45$\times$60s    	&	18.30   $\pm$ 0.09  	&	19.79 	&	\textcolor{black}{Lisnyky-AZT-8}     & this work  & MUPHOTEN-force,     \sa{calib. ps1/i}   VETO     \\
2022-10-13T01:49:56	&	59865.1248                    	&	3.5713              	&	$I_c$ 	&	23$\times$300s      	&	18.95  $\pm$ 0.12  	&	19.7 (5$\sigma$) 	&	\textcolor{black}{KNC-C11-FREE}   & this work & \sc{STDpipe}           \\
2022-10-15T18:44	&	59867.8639                    	&	6.3104              	&	$I_c$     	&	120$\times$60s   	&	19.77  $\pm$ 0.17  	&	19.0 	&	\textcolor{black}{Lisnyky-AZT-8}     & this work    &   \sc{Muphoten}         \\
2022-10-24T23:01	&	59877.0383                    	&	15.4848             	&	$I_c$     	&	685$\times$10s   	&	-	&	19.8 	&	\textcolor{black}{VIRT}          & this work        & \sc{Muphoten}
\\
\hline
%\multicolumn{10}{c}{$z^\prime$-band} \\
%\hline
2022-10-09T18:29	&	59861.7701                    	&	0.2167              	&	$z^\prime$ 	&	6$\times$60s      	&	14.89  $\pm$ 0.03  	&	-  	&	MeerLICHT      & \cite{2022GCN.32646....1D}  & -             \\ %off strange results
2022-10-10T12:25	&	59862.5174                    	&	0.9639              	&	$z^\prime$ 	&	2$\times$150s       	&	16.6   $\pm$ 0.09  	&	-   	&	SLT-40         & \cite{2022GCN.32667....1C} &    -         \\ %ok checked
2022-10-10T17:26	&	59862.7264                    	&	1.1729              	&	$z^\prime$ 	&	15$\times$30s   	&	16.87  $\pm$ 0.05  	&	19.8   	&	 AZT-20      & \cite{2022GCN.32769....1B} & -              \\ %checked sarah
2022-10-10T17:28	&	59862.7278                    	&	1.1743              	&	$z^\prime$ 	&	600s       	&	16.81  $\pm$ 0.01  	&	-   	&	RTT-150      &\cite{2022GCN.32743....1B}   & -                 \\ % ok checked
2022-10-10T17:15	&	59862.728                     	&	1.1745              	&	$z^\prime$ 	&	10$\times$80s    	&	16.97  $\pm$ 0.06  	&	20.3  	&	\textcolor{black}{KAO}     & this work   & \sc{Muphoten}                \\
2022-10-10T21:13	&	59862.884                     	&	1.3306              	&	$z^\prime$ 	&	600s      	&	16.99  $\pm$ 0.01  	&	-   	&	RTT-150     &\cite{2022GCN.32743....1B}   & -                 \\ % ok checked
2022-10-11T00:50	&	59863.0347                    	&	1.4813              	&	$z^\prime$ 	&	-       	&	16.92  $\pm$ 0.05  	&	-   	&	BlackGEM     & \cite{2022GCN.32678....1G} &      -        \\
2022-10-11T16:59	&	59863.7076                    	&	2.1542              	&	$z^\prime$ 	&	600s       	&	17.69  $\pm$ 0.02  	&	-   	&	RTT-150        &\cite{2022GCN.32743....1B}   & -                \\ % ok checked
2022-10-11T21:07	&	59863.8799                    	&	2.3264              	&	$z^\prime$ 	&	600s       	&	17.72  $\pm$ 0.03  	&	-   	&	RTT-150         &\cite{2022GCN.32743....1B}   & -                \\ % ok checked
2022-10-12T02:40	&	59864.1111                    	&	2.5577              	&	$z^\prime$ 	&	-     	&	18.26 $\pm$ 0.01	&	-  	&	LBTO      &         \cite{2022GCN.32759....1S} & -       \\ %ok
2022-10-12T14:34	&	59864.6092	&	3.0557	&	$z^\prime$	&	-	&	$18.40\pm0.11$	&  -	&	GMG-Lijiang	&	\citep{2022GCN.32727....1M} & -               \\ %ok checked
2022-10-12T17:16	&	59864.7194                    	&	3.166               	&	$z^\prime$ 	&	600s       	&	18.2   $\pm$ 0.04  	&	-   	&	RTT-150         &\cite{2022GCN.32743....1B}   & -                 \\ % ok checked
2022-10-12T17:48	&	59864.7417                    	&	3.1882              	&	$z^\prime$ 	&	600s       	&	18.19  $\pm$ 0.05  	&	-  	&	RTT-150        &\cite{2022GCN.32743....1B}   & -                 \\ % ok checked
2022-10-12T18:21	&	59864.7646                    	&	3.2111              	&	$z^\prime$ 	&	600s       	&	18.4   $\pm$ 0.08  	&	-   	&	RTT-150        &\cite{2022GCN.32743....1B}   & -                \\ % ok checked
2022-10-12T18:53	&	59864.7868                    	&	3.2333              	&	$z^\prime$ 	&	600s       	&	18.26  $\pm$ 0.03  	&	-   	&	RTT-150        &\cite{2022GCN.32743....1B}   & -                \\ % ok checked
2022-10-12T19:25	&	59864.809                     	&	3.2556              	&	$z^\prime$ 	&	600s       	&	18.23  $\pm$ 0.03  	&	-   	&	RTT-150          &\cite{2022GCN.32743....1B}   & -               \\ % ok checked
2022-10-12T19:40	&	59864.8194                    	&	3.266               	&	$z^\prime$ 	&	2100s       	&	18.35  $\pm$ 0.13  	&	-   	&	OHP             &  \cite{2022GCN.32753....1S} & \sc{STDpipe}          \\ % checked damien
2022-10-12T19:57	&	59864.8312                    	&	3.2778              	&	$z^\prime$	&	600s       	&	18.23  $\pm$ 0.04  	&	-   	&	RTT-150          &\cite{2022GCN.32743....1B}   &         -         \\ % ok checked
%2022-10-12T19:40	&	59864.8194                    	&	3.266               	&	sdssz 	&	2$\times$900     	&	18.35  $\pm$ 0.13  	&	0.0   	&	SVOM-OHP           &  - & calib. PS1               \\ %ok checked
2022-10-12T20:35	&	59864.8576                    	&	3.3042              	&	$z^\prime$ 	&	600s       	&	18.3   $\pm$ 0.04  	&	-  	&	RTT-150       &  \cite{2022GCN.32752....1B} &  -              \\ %ok checked
2022-10-12T21:08	&	59864.8806                    	&	3.3271              	&	$z^\prime$   	&	600s       	&	18.18  $\pm$ 0.04  	&	-   	&	RTT-150   &   \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T17:15	&	59865.7188                    	&	4.1653              	&	$z^\prime$ 	&	600s       	&	18.63  $\pm$ 0.05  	&	-   	&	RTT-150    & \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T17:47	&	59865.741                     	&	4.1875              	&	$z^\prime$ 	&	600s       	&	18.76  $\pm$ 0.05  	&	-   	&	RTT-150   & \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T18:19	&	59865.7632                    	&	4.2097              	&	$z^\prime$ 	&	600s       	&	18.69  $\pm$ 0.04  	&	-   	&	RTT-150    &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T17:51	&	59865.7705                    	&	4.217               	&	$z^\prime$ 	&	21$\times$110s   	&	18.90   $\pm$ 0.16  	&	19.8  	&	\textcolor{black}{KAO}    & this work    & \sc{Muphoten}               \\
2022-10-13T18:52	&	59865.7861                    	&	4.2327              	&	$z^\prime$ 	&	600s       	&	18.75  $\pm$ 0.04  	&	-   	&	RTT-150      &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T19:24	&	59865.8083                    	&	4.2549              	&	$z^\prime$ 	&	600s       	&	18.74  $\pm$ 0.05  	&	-   	&	RTT-150    &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T19:57	&	59865.8312                    	&	4.2778              	&	$z^\prime$ 	&	600s       	&	18.83  $\pm$ 0.05  	&	-   	&	RTT-150    &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T20:32	&	59865.8556                    	&	4.3021              	&	$z^\prime$ 	&	600s       	&	18.74  $\pm$ 0.05  	&	-   	&	RTT-150  &  \cite{2022GCN.32752....1B} & -               \\ %ok checked
2022-10-13T21:06	&	59865.8792                    	&	4.3257              	&	$z^\prime$ 	&	600s       	&	18.71  $\pm$ 0.06  	&	-   	&	RTT-150    &  \cite{2022GCN.32752....1B} & -             \\ %ok checked
2022-10-14T12:12	&	59866.5106	&	4.9571	&	$z^\prime$	&	-	&	$19.21\pm0.12$	&  -	&	GMG-Lijiang	&	\citep{2022GCN.32727....1M} & -               \\ %ok checked
2022-10-15T06:34	&	59867.2736                    	&	5.7202              	&	$z^\prime$	&	-      	&	19.39  $\pm$ 0.05  	&	-   	&	Faulkes     & \cite{2022GCN.32771....1S} &  -               \\ %ok checked
2022-10-15T16:08	&	59867.6722                    	&	6.1188              	&	$z^\prime$ 	&	15$\times$60s     	&	19.31  $\pm$ 0.08  	&	21.0 (3$\sigma$)  	&	AZT-20    & \cite{2022GCN.32769....1B} & - \\%ok checked
2022-10-22T16:22	&	59874.7375                    	&	13.184              	&	$z^\prime$ 	&	20$\times$240s   	&	-	&	20.4  	&	\textcolor{black}{KAO}    & this work    &\sc{Muphoten}               \\
2022-10-29T06:32	&	59881.2843                    	&	19.7308             	&	$z^\prime$ 	&	4$\times$260s    	&	21.01  $\pm$ 0.08  	&	24.0  	&	\textcolor{black}{CFHT-Megacam}    & this work & \sc{Muphoten}          \\ %checked
\hline
%\multicolumn{10}{c}{No filter} \\
%\hline                
2022-10-09T15:30	&	59861.6458                    	&	0.0924              	&	Clear 	&	180s       	&	15.5   $\pm$ 0.1   	&	-   	&	SCT   & \cite{2022GCN.32649....1O} & -               \\
2022-10-09T15:49	&	59861.659                     	&	0.1056              	&	Clear 	&	180s       	&	15.6   $\pm$ 0.1   	&	-   	&	SCT  & \cite{2022GCN.32649....1O} & -               \\
2022-10-09T17:14	&	59861.7181                    	&	0.1646              	&	Clear 	&	180s       	&	15.9   $\pm$ 0.1   	&	-   	&	SCT  & \cite{2022GCN.32649....1O} & -               \\
2022-10-09T18:44	&	59861.7806                    	&	0.2271              	&	Clear 	&	$\times$60s       	&	16.21  $\pm$ 0.11  	&	-   	&	BOOTES-2  & \cite{2022GCN.32644....1H} &  -\\
2022-10-10T19:29	&	59862.8257                    	&	1.2722              	&	Clear 	&	20$\times$60s    	&	18.52  $\pm$ 0.06  	&	19.5 	&	\textcolor{black}{MOSS}     & this work  & \sc{Muphoten}        \\
2022-10-10T19:31 & 59862.8490 & 1.2955 & $L$ & 34$\times$180s & 18.38 $\pm$ 0.25 & 20.2 (3$\sigma$) & \textcolor{black}{KNC-HAO} & this work & \sc{Muphoten} \\
2022-10-10T21:48:00	&	59862.9188                    	&	1.3652              	&	$CR$	&	  10$\times$180s    	&	18.76  $\pm$ 0.14  	&	19.2 (5$\sigma$) &	\textcolor{black}{KNC-MSXD}     & this work  & \sc{STDpipe}              \\
2022-10-11T16:33	&	59863.7069                    	&	2.1535              	&	Clear 	&	10$\times$150s   	&	-	&	17.5 	&	\textcolor{black}{SNOVA}           & this work   & \sc{Muphoten}        \\
2022-10-11T18:29:21	& 59863.7707                    	&	2.2172              	&	$CR$	&	  2$\times$30s    	&	-  	&	18.3 (5$\sigma$) &	\textcolor{black}{KNC-Montarrenti}     & this work  & \sc{STDpipe}              \\
2022-10-11T18:24:14	&	59863.7825                    	&	2.2290              	&	$CR$	&	  15$\times$180s    	&	19.22  $\pm$ 0.08  	&	20.3  &	\textcolor{black}{KNC-MSXD}     & this work  & \sc{STDpipe}              \\
2022-10-11T18:27:11	& 59863.8203                    	&	2.2668              	&	$L$ 	&	3$\times$2960s      	&	-	&	19.7 (5$\sigma$) 	&	\textcolor{black}{KNC-COK26}      & this work & \sc{STDpipe}           \\
%2022-10-11T18:46	&	59863.7819                    	&	2.2285              	&	Clear 	&	\sa{1$\times$0 s}      	&	19.13  $\pm$ 0.08  	&	20.3  	&	\textcolor{black}{KNC-SERR}     & this work       & \sa{STDPIPE-force?}         \\ % damien checked
2022-10-12T13:56	&	59864.5979                    	&	3.0445              	&	Clear 	&	10$\times$150s   	&	-	&	19.1 	&	\textcolor{black}{SNOVA}          & this work    & \sc{Muphoten}        \\
2022-10-14T18:17:29	&	59866.7944                    	&	5.2409              	&	$CR$	&	  31$\times$180s    	&	20.63  $\pm$ 0.11  	&	21.3 (5$\sigma$) &	\textcolor{black}{KNC-MSXD}     & this work  & \sc{STDpipe}             \\
2022-10-14T20:13:33	&	59866.8768                    	&	5.3233              	&	$CR$	&	 180$\times$32s    	&	20.46  $\pm$ 0.14  	&	21.0 (5$\sigma$) &	\textcolor{black}{KNC-T-CAT}     & this work  & \sc{STDpipe}             \\
2022-10-15T19:17:26 &	59867.8329                   	&	6.2795              	&	$CR$	&	  28$\times$180s    	&	20.75  $\pm$ 0.13  	&	21.3 (5$\sigma$) &	\textcolor{black}{KNC-MSXD}     & this work  & \sc{STDpipe}             \\
\hline
\end{tabular}}
\end{table*}

%2022-10-11T18:14:21 &    59863.75996527778              &   2.2065                  &   I       &   -       &   18.19   &   AbAO    %52$\times$60s

%2022-10-10T15:53:44 &   59862.662314814814              &   1.10885                &    Rc      &   19.27  $\pm$ 0.26   &   18.35   &   ShAO    %15$\times$90 s
%2022-10-10T15:58:41 &   59862.66575231482               &   1.11229                &    V       &   19.85  $\pm$ 0.37   &   19.50   &   ShAO    %25$\times$120 s

\end{center}

==> GRB221009A - Afterglow - APJL soumission(1)/extrafigures.tex <==
%\subsection{\textbf{Figures related to the multi-wavelength of the afterglow}}

\begin{figure*}%[!th]
\centering
\includegraphics[width=\textwidth]{figures/GRB221009A_LC_Fit2BPL.png}
  \caption{UVOIR light curve of GRB 221009A \textbf{(see section "Empirical light curve analysis)}. The magnitudes, expressed in the Vega system, are corrected for the SF11 galactic extinction. The break slope is at $\sim$ 0.6 d post GRB trigger time between $\alpha_1$ and $\alpha_2$.}
   \label{fig:LC_ALL}
\end{figure*}




\begin{figure}[t]
\centering
\includegraphics[width=0.55\columnwidth]{figures/GRB221009A_SF11_all_models_bestfitlcs_alldata_selected_filters_highlight_GRANDMA.pdf}
  \caption{ \texttt{NMMA} - Observational data (\textit{Extended} data) and best-fit light curves of selected filters for the NMMA analysis using the SF11 extinction and the four employed jet structures. The X-ray bands are shown in $\mu$Jy and the rest of the bands are shown in AB magnitude. In the optical band, the \textit{GRANDMA} data points are shown in orange.}
   \label{fig:NMMA_light curve}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/grb221009a_SF11_common_parameters_corner_no_numbers.pdf}
  \caption{ \texttt{NMMA} - Posterior distribution (shown are 90\% confidence intervals) for our selected data sets when using different jet models of \texttt{afterglowpy} analyzing the \textit{Extended} data.}
  \label{fig:NMMA_corner}
\end{figure*}

==> SED_results.tex <==
\renewcommand{\arraystretch}{1.4}
\begin{longtable}{cccccccc}
    \label{Table:host220427A}
	\caption[Table]{Summary of SED fitting results. (1) stellar mass in log scale, (2) SFR in log scale, (3) amount of dust attenuation in the V band, (4) metallicity, (5) age weighted by stellar mass, (6) attenuation curve slope for stellar continuum, (7) AGN fraction, (8) mass fraction of the late burst population.} \\ \hline
	%\label{tab:GRBHs_results}
    log$_{10}$(M$_{\star}$) & log$_{10}$(SFR) & A$_V$ & $Z$ & t$_{mass}$ & $\delta$ & $f_{agn}$ & $f_{burst}$ \\
    
	[M$_{\sun}$] & [M$_{\sun}$ yr$^{-1}$] & mag & & Myrs & & & \\ \hline
	\endfirsthead %\hline
$10.62_{-0.32}^{+0.18}$ & $1.89_{-nan}^{+0.31}$ & $1.32\pm0.51$ & $0.004_{-0.004}^{+0.007}$ & $802\pm668$ & $-0.60\pm0.30$ & $0.03_{-0.03}^{+0.06}$ & $0.08_{-0.08}^{+0.08}$ \\ \hline

\end{longtable}

==> cigal_params.tex <==
\begin{table}
	\renewcommand{\arraystretch}{1.2}
	\centering
	\caption{Input parameters for SED fitting with CIGALE}
	\label{Table:paramshost220427A}
	\begin{tabular}{c c c}
	\hline
	Parameter & Symbol & Range \\
	\hline\hline
	{\textbf{Delayed star formation history $+$ recent burst}}\\
	
	Age of the main stellar population & $t_0$ &  200, 500, 1000, 2000, 3000 \,Myrs \\
	E-folding time of the main stellar population model & $\tau$ &  200, 500, 1000, 2000, 3000, 5000, 7000, 10000  Myrs\\
	Mass fraction of the late burst population & $f_{burst}$ &  0.0, 0.1, 0.2\\
	Age of the late burst & $t_b$ &  20.0, 50.0, 100.0, 200.0\\
	E-folding time of the late starburst population & $\tau_{b}$ &  50.0\\
	%Age of the late starburst population & $t_{\rm b}$ &  1, 3, 5, 10, 15, 20, 30, 40, 50, 75, 100 \,Myrs \\
	%e-folding time of the late starburst population model & $\tau_{\rm b}$ &  50, 50000\,Myrs \\
	%Stellar mass fraction due to the burst & $f_{\rm b}$ &  0, 0.01, 0.03, 0.05, 0.075, 0.1, 0.15, 0.20\\
	\hline
	Metallicity $^1$ & $Z$ & 0.0001, 0.008, 0.02\\
    \hline
	{\textbf{Dust attenuation}}\\
	Color excess for nebular emission $^2$ & $\rm E(B-V)_{lines}$ & 0.01, 0.25, 0.5, 0.75, 1.0, 1.25, 1.5, 1.75, 2.0, 2.25, 2.5, 2.75, 3.0 \\
	Ratio of color excess & $\cfrac{E(B-V)_{stars}}{E(B-V)_{lines}}$ & 0.44 \\
	Attenuation curve slope for stellar continuum & $\delta$ & -1, -0.7, -0.4, -0.1, 0.2, 0.5, 0.7\\
	\hline
	{\textbf{AGN$^4$}}\\
	Slope of the power law & $\alpha$ & 2.0\\
	AGN fraction & $f_{agn}$ & 0.0, 0.1, 0.2 \\
	\hline
	Redshift & $z$ & 0.8159 \\
	\hline	
	\hline
	\end{tabular}
	\begin{flushleft}
      \small
      \item $^1$ {$Z$=0.02 being the solar metallicity}
      \item $^2$ {$\rm E(B-V)_{lines}$ is the color excess between the B and V bands applied on the nebular emission lines.}
      \item $^3$ {M$_d$ corresponds to the dust mass heated by the the radiation field intensity U. $\alpha_{IR}$ is fixed to 2 when no IR detection is available.}
      \item $^4$ {Parameters of the dale2014 model \cite{Boquien2019}.}
    \end{flushleft}

\end{table}
